MAST: A Memory-Augmented Self-supervised Tracker

Recent interest in self-supervised dense tracking has yielded rapid progress, but performance still remains far from supervised methods. We propose a dense tracking model trained on videos without any annotations that surpasses previous self-supervised methods on existing benchmarks by a significant margin (+15%), and achieves performance comparable to supervised methods. In this paper, we first reassess the traditional choices used for self-supervised training and reconstruction loss by conducting thorough experiments that finally elucidate the optimal choices. Second, we further improve on existing methods by augmenting our architecture with a crucial memory component. Third, we benchmark on large-scale semi-supervised video object segmentation(aka. dense tracking), and propose a new metric: generalizability. Our first two contributions yield a self-supervised network that for the first time is competitive with supervised methods on standard evaluation metrics of dense tracking. When measuring generalizability, we show self-supervised approaches are actually superior to the majority of supervised methods. We believe this new generalizability metric can better capture the real-world use-cases for dense tracking, and will spur new interest in this research direction.

==> sec/exp_v0.tex <==
%!TEX root=../egpaper_for_review.tex
\section{Experiments}
% As a fair comparison, 
% we pursue minimal changes made to the baseline systems~\cite{Lai19}, 
% and pinpoint the keys to build dense tracking systems purely based on self-supervised learning from videos.
% ===============
\input{./tables/davis-2017.tex}
We benchmark our model on two public benchmarks:
DAVIS-2017~\cite{Pont-Tuset17}  and the current largest video segmentation dataset, YouTube-VOS~\cite{Xu18}.
For both datasets,
a ground truth instance segmentation mask is given for the first frame, 
and the objective is to propagate the mask to subsequent frames.
In Section~\ref{sec:davis},  
we report performance of our full model and several ablated models on DAVIS benchmark.
Next, in Section~\ref{sec:youtube_vos}, we analyze the \emph{generalizability} of our model by benchmarking on the large-scale YouTube-VOS dataset.

\vspace{3pt}
\par \noindent \textbf{Standard evaluation metrics.} 
We use region similarity~($\mathcal{J}$) and contour accuracy~($\mathcal{F}$) to evaluate the tracked instance masks~\cite{Perazzi16}.

\vspace{3pt}
\par \noindent \textbf{Generalizability metrics} 
In order to demonstrate the generalizability of tracking algorithms under category-agnostic scenarios,
\ie~the categories in training set and testing set are disjoint,
YouTube-VOS also explicitly benchmarks the performances on unseen categories.
We therefore evaluate a generalization gap in Section~\ref{sec:gen}, 
which is defined as the average performance difference between seen and unseen object classes:
\begin{align}
\text{Gen. Gap} = \frac{(\mathcal{J}_{seen} - \mathcal{J}_{unseen}) + (\mathcal{F}_{seen}  - \mathcal{F}_{unseen})}{2}
\end{align}

% ---------------
\subsection{Video Segmentation on DAVIS-2017}
\label{sec:davis}
\subsubsection{Main results}
% ---------------
In Table~\ref{table:davis_1}, 
we compare MAST with previous approaches on the DAVIS-2017 benchmark. 
Two phenomena can be observed:
\emph{first},
our proposed model has clearly dominated all the other self-supervised methods,
surpassing previous state-of-the-art CorrFlow by a significant margin~($65.5$ vs $50.3$ on $\mathcal{J}$\&$\mathcal{F}$).
\emph{Second}, 
despite only using ResNet18 as feature encoder,
our model trained with self-supervised learning can still surpass some of the results by heavily supervised learning.

% \subsubsection{Qualitative Results}
% % ===============
% As shown in Figure~\ref{fig:qualitative} and Figure~\ref{fig:qualitative_2}, 
% SMAT can propagate the segmentation mask through sequences even in the presence of large scale variation from camera motion, 
% and large object deformation. 

% --------------------
\begin{figure*}[!htb]
  \centering
%  % Requires \usepackage{graphicx}
  \includegraphics[width=\textwidth]{figures/qualitative_with_others_v2.pdf}
  \vspace{-3pt}
  \caption{Our method vs. previous self-supervised methods. 
  Other methods show systematic errors in handling occlusions. Row 1: The dancer undergoes large self-occlusion. %, causing other methods to lose track (TC and CF) or over segment (OSVOS).
  Row 2: The dog is repeatedly occluded by poles. %, and other methods show different degrees of loss in track (especially VC and TC).
  Row 3: Three women reappear after being occluded by the man in the foreground.% Three other propagation-based methods without memory-augmentation (VC,TC,CF) fail severely.
  }
    \vspace{-1.5em}

  \label{fig:qualitative_2}
\end{figure*}
%
% --------------------

% ===============
\vspace{-5pt}
\subsubsection{Ablation Studies}
\label{exp:ablation}

To examine the effects of different components, 
we conduct a series of ablation studies by removing one component at a time.
All models are trained on OxUvA~(except the analysis on dataset), 
and evaluated on the dense tracking task~(semi-supervised video segmentation on DAVIS-2017) \emph{without} any finetuning.  
\\[-5pt]
% ===============
\input{tables/ablation.tex}
% ===============
% --------------------
\par \noindent  \textbf{Choice of color spaces.}
% --------------------
As shown in Table~\ref{tab:abl_color}, 
we perform different experiments with input frames transformed into different color spaces, \eg~RGB, $Lab$ or HSV.
We find that the MAST model trained with $Lab$ color space always outperforms the other color spaces,
validating our conjecture that dropout in a decorrelated color space leads to better feature representations for self-supervised dense tracking, as explained in Section~\ref{sec:color}.
Additionally, 
we compare our default setting with a model trained with cross-color space matching task~(shown in Table~\ref{tab:abl_cross_color}).
That means to use a different color space for the input and the training objective, 
\eg~input frames are in RGB, and loss function is defined in $Lab$ color space.
Interestingly, the performance drops significantly, 
we hypothesis this can attribute to the fact that all RGB channels include a representation of brightness,
making it highly correlate to the luminance in $Lab$, 
therefore acting as a weak information bottleneck.
\\[-10pt]
% % --------------------
\par \noindent  \textbf{Loss functions.}
% % --------------------
As a variation of our training procedure, 
we experiment with different loss functions: 
cross entropy loss on the quantized colors, and photometric loss with Huber loss.
As shown in Table~\ref{tab:abl_color}, 
regression with real-valued photometric loss surpasses classification significantly,
validating our conjecture that the information loss during color quantization ends up with inferior representations for self-supervised tracking~(as explained in Section~\ref{sec:training_signal}),
due to less discriminative training signals.
\\[-5pt]
% --------------------
\par \noindent  \textbf{Image feature alignment.}
% --------------------
To evaluate the alignment module proposed for aligning features with the original image, 
we compare it to direct bilinear image downsampling used by CorrFlow\cite{Lai19}. 
The result in Table~\ref{tab:abl_align} shows that our approach achieves about $2.2\%$ higher performance.  
\\[-5pt]

% --------------------
\par \noindent  \textbf{Dynamic memory by exploiting more frames.}
% --------------------
% {\color{red} TODO: make this clear}
We compare our default network with variants that have only short term memory or long term memory. 
Results are shown in Table~\ref{tab:abl_mem}.
While both short term memory and long term memory alone can make reasonable predictions,
the combined model achieves the highest performance.
The qualitative predictions~(Figures~\ref{fig:qualitative} and~\ref{fig:qualitative_2}) also confirm that the improvements come from reduced tracker drift.
For instance, when severe occlusion occurs, 
our model is able to attend and retrieve high-resolution information from frames that are temporally distant. In Fig.~\ref{fig:mem_perf}, we confirm that a 5-frame memory is optimal for our task.

% ===============
\begin{figure}[H]
  \centering
  \includegraphics[width=.45\textwidth]{figures/fig_mem_v1.pdf}
  \vspace{-2pt}
  \caption{\textbf{Optimal memory size}: 
  The performance of our model first increases when number of frame in memory grows. After memory reaches 5 frames, the performance plateaued. }
  \label{fig:mem_perf}
\end{figure}
% ===============
% hypothesize that since the tracked objects may often be occluded or deformed,
%it is unreasonable to force each ROI to share importance.
%Aggregating similarity across the temporal dimension alleviates the issue:
%ROIs that have low overall similarity are ignored by a global softmax operation.  
% \\[-5pt]
% --------------------
%\paragraph{Soft vs. Hard mask propagation}
% --------------------
%As shown in Table~\ref{tab:abl_prop}, 
%we show the soft mask propagation is beneficial.
% --------------------
% \par \noindent  \textbf{Choice of training data.}
% % --------------------
% As shown in Table~\ref{tab:abl_dataset}, 
% we train SMAT on different datasets: 
% ImageNet VID~\cite{Deng09}, OxUvA~\cite{Valmadre18}, and YouTube-VOS~\cite{Xu18} training splits.
% The model trained on ImageNet VID shows slightly worse performance on the dense tracking task,
% which we conjecture is because the dataset contains relatively short videos, 
% therefore fewer challenging scenarios that lead to tracker drift will appear, \eg~occlusion or disocclusion.
% Despite the small variation in performance, 
% the results still show that the proposed architecture and training scheme are generally successful and
% not due to well-selected training data.
% % ===============

\subsection{Youtube Video Object Segmentation}
\label{sec:youtube_vos}
We also evaluate the MAST model on the Youtube-VOS validation split~(474 videos with 91 object categories).
As no other self-supervised methods have been tested on the benchmark, 
we directly compare our results with supervised methods. 
As shown in Table~\ref{table:youtube_1}, 
our method achieves results comparable to many heavily supervised methods. 

% ===============
\input{tables/youtube-vos.tex}
% ===============
\subsubsection{Generalizability}
\label{sec:gen}
As another metric for evaluating category-agonostic tracking, 
the YouTube-VOS dataset has conveniently separate measures for seen and unseen object categories. 
We can therefore estimate testing performance on out-of-distribution samples to gauge the model's generalizability to more challenging, unseen, real-world scenarios. 
As seen from the last two columns, we rank second amongst all algorithms in unseen objects. 
In these unseen classes, 
we are even $3.9\%$ higher than the DAVIS 2018 and YouTube-VOS 2018 video segmentation challenge winner, 
PreMVOS\cite{Luiten18}, 
a complex algorithm trained with multiple large manually labeled datasets.
For fair comparison, 
we train our model only on the YouTube-VOS training set. We also re-train two most related self-supervised methods in the same manner as baselines. % (so the `Seen' and `Unseen' separation holds true to our model). 
Even learning from only a subset of all classes, 
our model generalizes well to unseen classes,
with a generalization gap (\ie the performance difference between seen and unseen objects) near zero ($0.4$). 
This gap is much smaller than any of the baselines ($\text{avg}=11.5$), 
suggesting a unique advantage to most other algorithms trained with labels. 

By training on large amount of unclassified videos, the feature extractor is learned without using any information of object classes. This means that the learned feature is more independent to a specific set of object class (\ie those in the training set). Therefore, the process is more close to an optimal ``universal feature extraction'', \ie features should contain less manual and hand-crafted information. Indeed, the only supervised algorithm that is comparable to our method in generalizability is OSVOS (2.7 \textit{vs.} 0.4). However, OSVOS uses the first image from the testing sequence to perform a costly one-shot fine-tuning. This is inferior to our algorithm, which has zero-shot generalization ability. 

Note our model also has a smaller generalization gap compared to other self-supervised methods as well. This further attesting to the robustness of its learned features, suggesting that our improved reconstruction objective is highly effective in capturing general features. 

%This could suggest that our model learns more class-agnostic features - making it another valuable aspect of our method.

==> sec/intro.tex <==
%!TEX root=../egpaper_for_review.tex

Although the working mechanisms of human visual system remain somewhat obscure at the level of neurophysiology, 
it is a general concensus that tracking objects is a fundamental ability that a baby starts developing since two to three months age~\cite{Brazelton66, Kremenitzer79, Hofsten82}. 
Similarly, in computer vision systems, 
tracking plays key roles in a large number of applications ranging from autonomous driving to video surveillance. 

% =========================
\begin{figure}[t]
\includegraphics[width=0.5\textwidth]{figures/fig1.pdf}
\centering
\vspace{-0.5cm}
\caption{Comparison with other recent works on the DAVIS-2017 benchmark, 
\ie dense tracking or instance-wise video segmentation given the first frame annotation.
The proposed dense tracking system achieves state-of-the-art performance among all self-supervised approaches,
even comparable to some approaches trained with heavy supervision with ImageNet, COCO, Pascal, DAVIS, Youtube-VOS.\\
\textbf{Notation}:
CorrFlow~\cite{Lai19}, CycleTime~\cite{Wang19}, mgPFF~\cite{Song19}, Colorization~\cite{Vondrick18},
OSVOS~\cite{Caelles17}, VideoMatch~\cite{Hu18}, RGMP~\cite{Oh18}, OnAVOS~\cite{Voigtlaender17}, 
OSMN~\cite{Yang18}, FAVOS~\cite{Cheng18}, OSVOS-S~\cite{Maninis18}, FEELVOS~\cite{Voigtlaender19}, 
DyeNet~\cite{Li18ECCV}, PReMVOS~\cite{Luiten18}.}
\label{fig:teaser}
\vspace{-10pt}
\end{figure}
% =========================

Given arbitrary objects defined in the first frame, 
a tracking algorithm aims to relocate the same object throughout the entire video sequence. 
In the literature, 
tracking can be cast into two categories:
One is typically termed Visual Object Tracking (VOT)~\cite{VOT_TPAMI}, 
the goal is to relocalize the objects with bounding boxes through the video;
The other one aims for more fine-grained tracking, \ie relocalize the objects with segmentation masks,
this is recently put in the name of Semi-supervised Video Object Segmentation (Semi-VOS)~\cite{Pont-Tuset17}.
In this paper, we focus on the latter case. 
To avoid abuse of terminology, this is termed as \emph{dense Tracking} from here on. 

% ===============
\begin{figure*}[!htb]
  \centering
%  % Requires \usepackage{graphicx}
  \includegraphics[width=.98\textwidth]{figures/qualitative_v3.pdf}
  \vspace{-3pt}
  \caption{Qualitative results from our \emph{self-supervised dense tracking model} on DAVIS-2017 and YouTube-VOS dataset. 
 The number on top left refers to the frame number in the video.
 For all examples, the mask for $0th$ frame is given, and the task is to track the objects along the video.
 Our self-supervised tracking model is able to deal with challenging scenarios, 
 such as large camera motion, occlusion and disocclusion, large deformation and scale variation.}
  \label{fig:qualitative}
\end{figure*}
% ===============
Extensive human annotations are required to achieve superior performance on dense tracking~(as shown in Figure~\ref{fig:teaser}),
for instance, an ImageNet~\cite{Deng09} pretrained ResNet is usually adopted as a feature encoder,
and further fintuned on a large number of images or frames with fine-grained, pixel-level segmentations, 
\eg COCO~\cite{Lin14}, Pascal~\cite{Everingham09a}, DAVIS~\cite{Pont-Tuset17} and YouTube-VOS~\cite{Xu18}.
Despite the rapid progress in dense tracking,
these supervised training seems very counter-intuitive when comparing with the development of human vision system.
It is known that human babies have already developed the ability for eye coordination and tracking by three months of age~\cite{Brazelton66, Kremenitzer79, Hofsten82}, 
in other words, 
the ability to track and follow slow-moving objects appears at a much earlier stage than being able to map objects to semantic meanings. 
With these evidences, it is unlikely the case that humans develop their tracking ability in a top-down manner, 
at least not at the early stage development of our vision systems.

In addition to the aforementioned approaches based on heavy supervision, 
several self-supervised methods~\cite{Vondrick18, Wang19, Lai19} have recently been proposed, 
leading more attractive directions for exploration since expensive semantic annotations are not required during training.
Unfortunately, none of the previous systems has demonstrated satisfactory results so far, 
they typically suffer from the problem from large deformation, fast motions, tracker drifting due to occlusions or disocclusions.
In this paper, we carefully examine the design choices in previous works~\cite{Vondrick18, Lai19}, 
pinpoint the potential flaws, and experimentally validate our conjectures to analyze the effects of core factors.

We make the following contributions:
First, 
we demontrate that channel dropout and jitterings are most effective
on $Lab$ color space, where the channels are decorrelated and reflect human perception. 
Second, to improve the training strategy, 
we spatially align the feature representation and downsampled image, 
train the models with photometric loss between the reconstructed and original frames,
naturally providing more discriminative training signals.
Third, we introduces a mechanism that allows hierarchical, dynamic memory mechanism.
To minimize the computational overhead and memory consumption,
we borrow the intuition from pre-attentive processing , 
\ie all available information in the previous video frames are coarsely processed, 
and information that has the highest salience or relevance is selected for further and more complete analysis by conscious (attentive) processing. 

We demonstrate that our method surpasses all existing self-supervised dense tracking methods by a significant margin on 
DAVIS-2017 and YouTube-VOS benchmarks~(Figure~\ref{fig:teaser}). 
Moreover, for the first time, 
we show that self-supervised learning on raw videos is able to produce competitive performance as those trained with heavy supervision.
While benchmarking on the unseen objects that not appearing in the training set, 
our model even outperform the heavily-engineered entries from the DAVIS competition winner,
demonstrating the usefulness and superior generalizability.
The goal of this paper is by no means to deny the necessity or the importance of supervised learning, 
instead, we try to demonstrate the potential of self-supervised dense tracking, 
and provide a strong baseline for future researches.

%On the other hand, state-of-the-art tracking by bounding box method typically adopt a siamese network based structure. 
%Such structure explores the translation-invariance property of CNNs and cast tracking into a similarity learning problem. 
%For example, [][] aims to compare an object template to sub-windows within the candidate image using shared-weight fully-convolutional conv-nets followed by a cross-correlation operation.

%In the same spirit of self-supervision, we propose a model that could be trained without any human supervision. 
%But we try to extend the previous methods by solving the aforementioned failure cases. Also, we propose a new memory mechanism to alliviate drifting and occlusion-related problems. As shown in Fig.~\ref{fig:teaser}, our model is able to achieve results comparable to many heavily supervised methods.



==> sec/intro_v2.tex <==
%!TEX root=../egpaper_for_review.tex

Although the working mechanisms of the human visual system remain somewhat obscure at the level of neurophysiology, 
it is a consensus that tracking objects is a fundamental ability that a baby starts developing at two to three months of age~\cite{Brazelton66, Kremenitzer79, Hofsten82}. 
Similarly, in computer vision systems, 
tracking plays key roles in a large number of applications ranging from autonomous driving to video surveillance. 

% =========================
\begin{figure}[t]
\includegraphics[width=0.5\textwidth]{figures/fig1.pdf}
\centering
\vspace{-0.5cm}
\caption{Comparison with other recent works on the DAVIS-2017 benchmark, 
\ie dense tracking or instance-wise video segmentation given the first frame annotation.
The proposed dense tracking system achieves state-of-the-art performance among all self-supervised approaches,
even comparable to some approaches trained with heavy supervision with ImageNet, COCO, Pascal, DAVIS, Youtube-VOS.\\
\textbf{Notation}:~CorrFlow~\cite{Lai19}, CycleTime~\cite{Wang19}, mgPFF~\cite{Song19}, Colorization~\cite{Vondrick18},
OSVOS~\cite{Caelles17}, VideoMatch~\cite{Hu18}, RGMP~\cite{Oh18}, OnAVOS~\cite{Voigtlaender17}, 
OSMN~\cite{Yang18}, FAVOS~\cite{Cheng18}, OSVOS-S~\cite{Maninis18}, FEELVOS~\cite{Voigtlaender19}, 
DyeNet~\cite{Li18ECCV}, PReMVOS~\cite{Luiten18}.}
\label{fig:teaser}
\vspace{-10pt}
\end{figure}
% =========================

Given arbitrary objects defined in the first frame, 
a tracking algorithm aims to relocate the same object throughout the entire video sequence. 
In the literature, 
tracking can be cast into two categories:
one is typically referred to as Visual Object Tracking (VOT)~\cite{VOT_TPAMI}, 
with the goal of relocalizing objects with bounding boxes throughout the video;
the other one aims for more fine-grained tracking, \ie relocalize the objects with pixel-level segmentation masks,
also known as Semi-supervised Video Object Segmentation (Semi-VOS)~\cite{Pont-Tuset17}.
In this paper, we focus on the latter case and refer to it as \emph{Dense Tracking} from here on. 

In order to achieve superior performance on such dense tracking task, 
recent methods usually require extensive manual annotations~(as shown in Figure~\ref{fig:teaser});
for instance, an ImageNet~\cite{Deng09} pre-trained ResNet is usually adopted as a feature encoder,
and further finetuned on a large number of images or frames with fine-grained, pixel-level semantic segmentation, 
\eg COCO~\cite{Lin14}, Pascal~\cite{Everingham09a}, DAVIS~\cite{Pont-Tuset17} and YouTube-VOS~\cite{Xu18}.
However, these supervised training schemes seem counter-intuitive when comparing to the development of the human vision system,
as human babies can track and follow slow-moving objects from two to three months of age, 
which is clearly a much earlier stage than being able to map objects to semantic meanings. 
With this evidence, 
it is unlikely the case that humans develop their tracking ability in a top-down manner~(supervised by semantics), 
at least not at the early stage development of the vision system.

% ===============
\begin{figure*}[!htb]
  \centering
%  % Requires \usepackage{graphicx}
  \includegraphics[width=.98\textwidth]{figures/qualitative_v3.pdf}
  \vspace{-3pt}
  \caption{\textbf{Train once, test on multiple datasets:}
Qualitative results from our \emph{self-supervised dense tracking model} on DAVIS-2017 and YouTube-VOS dataset. 
The number on the top left refers to the frame number in the video.
For all examples, the mask for $0th$ frame is given, and the task is to track the objects along with the video.
Our self-supervised tracking model is able to deal with challenging scenarios, 
such as large camera motion, occlusion and disocclusion, large deformation and scale variation.}
\label{fig:qualitative}
\end{figure*}
% ===============

In addition to the aforementioned approaches based on heavy supervision, 
several self-supervised methods~\cite{Vondrick18, Wang19, Lai19} have recently been proposed, 
leading to more attractive directions for exploration since expensive semantic annotations are not required during training.
Such self-supervised tracking algorithms have been proved possible without any finetuning.  
This differs from the self-supervised setting for other tasks, 
\eg~classification, which trains only the feature representation, 
and a final classification layer is still required to finetune on the full dataset with ground truth annotations. 
Self-supervised visual tracking algorithms\cite{Vondrick18,Wang19,Lai19,Wang19_Tracking}, 
on the other hand, are complete and do not require such a finetuning step.  

The most popular framework among these self-supervised tracking algorithms is based on feature similarity, 
\ie~label of the query pixel is assigned by the nearest reference pixels in the embedding space.
In this work, we argue in the same line and extend the idea of~\textit{correspondence flow} proposed by~\cite{Lai19}. 
Correspondence flow replaces traditional optical flow by relaxing the brightness constancy constraint and spatial smoothness,
allowing each query pixel to have correspondence with multiple reference pixels.
This representation turns out to be suitable for self-supervised dense tracking and has been shown to provide a huge performance gain over that based on optical flow. 

However, we identify a key issue of the method: 
the existing correspondence flow does not model large movement, 
since the query pixel can only look for similarities within a reference patch that is always placed around the query pixel. 
Motivated by this shortcoming, 
we add an offset to the representation and thus allow the patch to be non-locally placed, 
enabling the model to search for the reference patch dynamically.
We call this augmented representation, the \textit{non-local correspondence flow}. 

Building on our new non-local correspondence flow, 
we augment the tracking system proposed in \cite{Lai19} with a pre-attentive memory mechanism 
which allows to firstly make fixations to both long term and short term memories, 
and process the attended regions with a more complete analysis.
We show this is essential for dealing with the problems of large motion and occlusion in visual tracking, 
thus avoiding the complex training pipeline for handling tracker drift introduced in \cite{Lai19}. 
Our entire network, which we call \emph{Self-supervised Non-local Tracking Network (SNTNet)}, 
can be trained end-to-end on raw videos without any human annotation.

We evaluate SNTNet on multiple benchmarks for dense tracking with several compelling discoveries: 
First, our algorithm surpasses all existing self-supervised dense tracking methods by a significant margin on DAVIS-2017 ($13\%$) and YouTube-VOS ($20\%$) benchmarks, making SNTNet competitive with supervised methods. 
Second, we find that the model trained only on a small set of videos has already shown superior generalization capabilities on unseen objects and scenes. 
On the YouTube-VOS benchmark, we comfortably surpass PreMVOS~\cite{Luiten18}, 
the 2018 challenge winner algorithm trained with massive annotated datasets, on unseen object classes. 
Finally, we propose new training strategies with more effective losses and decorrelated color space,
which significantly improve the tracking performance, 
yielding state-of-the-art performance without using any human annotations.

==> sec/method_v0.tex <==
%!TEX root=../egpaper_for_review.tex
\section{Method}
% {\color{red} TODO: add overview: 1) background, 2) improvements, 3) tracker}
The proposed dense tracking system, 
MAST (Memory-Augmented Self-supervised Tracker), 
is a conceptually simple model for dense tracking that can be trained with self-supervised learning,
\ie \textbf{zero manual annotation} is required during training,
and an object mask is only required for the first frame during inference.
In Section~\ref{sec:background},
we provide relevant background of previous self-supervised dense tracking algorithms,
and termonologies that will be used  in later sections.

Next, in Section~\ref{sec:training_signal}, 
we pinpoint weaknesses in these works and propose improvements to the training signals.
Finally, in Section~\ref{sec:memory}, we propose memory augmentation as an extension to existing self-supervised trackers.

%
\subsection{Background}
\label{sec:background}
% {\color{red} Todo: make background section more concise, especially last paragraph.}
%\begin{figure}[!h]
%  \centering
%  \includegraphics[width=.45\textwidth]{figures/background.pdf}
%  \vspace{-2pt}
%  \caption{\textbf{Correspondence from frame reconstruction}: The correspondence can be learned from reconstructing target from the reference frame. After the correspondence is learned, it can be used to track arbitrary objects.}
%  \label{fig:background}
%\end{figure}

In this section,
we review previous works that are closely related~\cite{Vondrick18, Lai19}.
The goal of self-supervised tracking is to learn robust feature representations that enables robust correspondence matching.
During training, 
the proxy task is posed as reconstructing a target frame~($I_t$) by ``copying''~(linearly combining) pixels from $I_{t-1}$,
where the correspondence between pixels in target frame and reference frame is computed with \emph{Attention} mechanism. 
%a learned feature extractor (Fig.~3 encoder) produces representations suitable for correspondence matching are learned as a byproduct from \textit{frame reconstruction}. 

%This process can be understood in the general framework of (self-)attention~\cite{Vaswani17},
%that is designed for Seq2Seq problems:
%an input sequence (original video sequence), \eg~$S_{input}=\{I_t\}_{t=1}^n$
%is used to predict an output sequence (reconstructed video sequence), \eg~$S_{output}=\{\hat{I}_t\}_{t=1}^n$.

Specifically, a triplet~($\{Q_t, K_t, V_t\}$) exists for each input frame $I_t$, 
referring to \emph{Key}, \emph{Query}, and \emph{Value}.
In order to reconstruct a pixel $i$ in the $t$-th frame~($\hat{I^i_t}$),
an \textit{Attention} mechanism is used for  \emph{soft-copying} pixels from a subset of previous frames in the original sequence,
this procedure is formalized as
\begin{align} 
\label{eq:attention}
  \hat{I^i_t} = \sum _{j} A^{ij}_{t} V^j_{t-1} \\
\label{eq:affinity}
  A^{ij}_t =  \frac{exp\langle\ Q_t^i,K_{t-1}^j\rangle}{\sum_p exp\langle\ Q_t^i,K_{t-1}^p\rangle}
\end{align}

\noindent where $\langle\cdot,\cdot\rangle$ refers to the dot product between two vectors,
and $A_t$ is the affinity matrix representing the feature similarity between pixel $I^i_t$ and $I^j_{t-1}$.
In these works, query~(Q) and key~(K) are feature representations computed by 
passing the target frame $I_t$ to the same deep ConvNet $\Phi(\cdot; \theta)$, 
\ie $Q_t = K_t = \Phi(I_t; \theta)$. 
Value~(V) is the raw reference frame~($I_{t-1}$) during the training stage, 
and instance segmentation mask during inference.


% Here, the underlying assumption is that the pixel in the current frame can be reconstructed by a linear combination of all pixels in the previous frame. 
% As an improvement, \cite{Lai19} argues that this assumption is unnecessary because objects always move locally between frames. 
% Therefore, they propose to use \textit{correspondence flow} to 
% reconstruct each query pixel by linear combinations of the reference pixels in a window with restricted size.
% This representation has been shown to achieve state-of-the-art performance in self-supervised dense tracking.

A key element in self-supervised learning is the \emph{information bottleneck},
or the decision of what input information to withhold to learn a good feature representation
and to avoid learning trivial solutions.
For example, in the frame reconstruction task,
an obvious shortcut is that the pixel in $I_t$ can learn to match any pixel in $I_{t-1}$ with the \emph{exact same color}, 
yet not necessarily share any semantic similarity.
%Another concern is to avoid trivial solutions during training; in other words, if training is done na\"ively,
%it is not guaranteed to obtain feature representations for high-quality correspondence matching.
%An obvious shortcut is that the pixel in $I_t$ can learn to match any pixel in $I_{t-1}$ with the \emph{exact same color}, yet not necessarily share any semantic similarity.
To circumvent such learning shortcuts,
Vondrick \etal~\cite{Vondrick18} intentionally drop the color information from the input frames.
Lai and Xie~\cite{Lai19} further show that a simple channel dropout can be effective.

% With the learnt affinity matrix,
% the downstream dense tracking is therefore posed as mask propagation from $M_{t-1}$~(instance mask of $I_{t-1}$):
% \begin{align}
% M^{i}_t = \sum_{j} A_{ij} M^j_{t-1}
% \label{eq:prop}
% \end{align}

% $\Phi(\cdot; \theta)$ is a deep ConvNet.

% the query~(Q) refers to the pixelwise feature representation computed from the current frame, \ie $f_t$;
% the key~(K) refers to the feature representation of the reference frame, \ie $f_{t-1}$,
% while value~(V) denotes the raw reference frame~($I_{t-1}$) during the training stage, 
% and instance segmentation mask~($M_{t-1}$) during inference.
% For simplicity, we will stick on this set of notations in the following sections.

% % Formally,
% % assume we are given two frames from a video~$I_{t-1}$ and $I_t$~($t-1$ and $t$ refer to the time point).
% % ,
% % then a feature encoder $f$ is parametrized by a ConvNet, denoted as $\Phi(\cdot; \theta)$:
% % \begin{align}
% % f_{t-1}, f_t = \Phi(I_{t-1}; \theta), \Phi(I_t; \theta)
% % \end{align}
% % The goal is to enable every pixel in $I_t$ to find its counterpart in frame $I_{t-1}$,
% % which share the same semantics.
% % Notice objects generally move smoothly and appearance will not change abruptly, so we assume frame $I_t$ can be reconstructed purely by ``copying'' pixels from $I_{t-1}$,
% % correspondence matching has been learnt.
% % In \cite{Vondrick18}, this intuition is formalized as :
% \begin{align}
% \hat{I^i_t} = \sum _{j} A_{ij} I^j_{t-1} \text{\hspace{.25cm}
% where\hspace{.1cm}} A_{ij} =  \frac{exp\langle\ f^i_t,f^j_{t-1}\rangle}{\sum_k exp\langle\ f^i_t,f^k_{t-1}\rangle}
% \label{eq:affinity}
% \end{align}
% %
% where $\hat{I^i_t}$ refers to the reconstructed frame for $I_t$,
% $\langle\cdot,\cdot\rangle$ refers to the dot product between two vectors,
% and $A$ is the affinity matrix with each element representing the pairwise pixel similarity,
% \eg\ $A_{ij}$ denotes the correspondence between pixel $I^i_t$ and $I^j_{t-1}$. 
% The underlying assumption is that the pixel in the current frame can be reconstructed by a linear combination of all pixels in the previous frame. 
% As an improvement, \cite{Lai19} argues that this assumption is unnecessary because objects always move locally between frames, 
% \ie the natural spatial-temporal consistency in videos. 
% Therefore, they propose to use \textit{correspondence flow} that 
% reconstructs each query pixel by linear combinations of the reference pixels in a window with restricted size.
% This representation has been shown to yield state-of-the-art performance in self-supervised dense tracking.

% Another concern is to avoid trivial solutions during training, in other words, if training is done na\"ively,
% it is not guaranteed to obtain feature representations for high-quality correspondence matching.
% An obvious shortcut is that the pixel in $I_t$ can learn to match any pixel in $I_{t-1}$ with the \emph{exact same color}, yet not necessarily share any semantic similarity.
% To circumvent such learning shortcuts,
% Vondrick \etal~\cite{Vondrick18} intentionally drop the color information from the input frames.
% Lai and Xie~\cite{Lai19} further show that a simple channel dropout can be effective.

% With the learnt affinity matrix,
% the downstream dense tracking is therefore posed as mask propagation from $M_{t-1}$~(instance mask of $I_{t-1}$):
% \begin{align}
% M^{i}_t = \sum_{j} A_{ij} M^j_{t-1}
% \label{eq:prop}
% \end{align}

% Note, this architecture design can also be categorized as a simplified version of attention-based models.
% In Transformer~\cite{Vaswani17}, the encoded representations are represented as key-value pairs~(K,V), 
% during decoding, the previous output is compressed into a query~(Q), 
% and the next output is produced by using this query to retrieve relevant information from the set of keys and values.
% While in the aforementioned case for correspondence learning,
% the query~(Q) refers to the pixelwise feature representation computed from the current frame, \ie $f_t$;
% the key~(K) refers to the feature representation of the reference frame, \ie $f_{t-1}$,
% while value~(V) denotes the raw reference frame~($I_{t-1}$) during the training stage, 
% and instance segmentation mask~($M_{t-1}$) during inference.
% For simplicity, we will stick on this set of notations in the following sections.

% ------------------
\subsection{Improved Reconstruction Objective} 
\label{sec:training_signal}
% ------------------
In this section,
we reassess the choices made in previous self-supervised dense tracking works and propose improvements.
%we discuss potential directions for improving training signals in self-supervised dense tracking.
%To analyze the core factors,
For a fair comparison,
we adopt the exact same architecture~(ResNet18) from~\cite{Lai19}.
% ------------------
\vspace{-5pt}
\subsubsection{Decorrelated Color Space}
\label{sec:color}
% ------------------
Extensive experiments in the human visual system have shown that colors can be seen as combinations of the primary colors,
namely red (R), green (G) and blue (B).
For this reason, 
most of the cameras and emissive color displays represent pixels as a triplet of intensities:~$(R,G,B) \in \mathcal{R}^3$.
However, as shown in Figure~\ref{fig:color}, 
a disadvantage of the RGB representation is that the channels tend to be extremely correlated~\cite{Reinhard01}.
In this case, 
the channel dropout proposed in~\cite{Lai19} is unlikely to behave as an effective information bottleneck,
since the dropped channel can almost always be determined by one of the remaining channels.

% ===============
\begin{figure}[!h]
  \centering
  \includegraphics[width=.45\textwidth]{figures/colorspace_v7.pdf}
  \vspace{-2pt}
  \caption{Correlation between channels of RGB and $Lab$ colorspace. 
We randomly take $100000$ pixels from a sequence~(snowboard) in the DAVIS dataset and plot the relative relationships between RGB channels. This phenomena generally holds for all natural images~\cite{Reinhard01}, 
due to the fact that all of the channels include a representation of brightness.
Values are normalized for visualization purposes.}
  \label{fig:color}
\end{figure}
% ===============

To remedy this limitation,
we hypothesize that dropout in the decorrelated representations~(\eg~$Lab$) 
would force the model to learn invariances suitable for self-supervised dense tracking;
\ie if the model cannot predict the missing channel from the observed channels,
it is forced to learn a more robust representation rather than relying on local color information.
%for instance, if the color of one input channel is unpredictable from the others, 
%yet the model is still capable to matching the correspondence and copying colors from a reference frame, 
%it must have learnt more robust representations that are invariant to the low-level colors.
%In Section~\ref{exp:ablation}, 
%we validate our conjecture that channel-wise dropout
%are indeed more effective on input frames represented in the $Lab$ color space,
%which separates luminance and chrominance, resulting in low mutual information.

% ------------------
\vspace{-5pt}
\subsubsection{Classification vs. Regression}
\label{sec:loss}
% ------------------
In the recent literature on colorization and generative models~\cite{Zhang16_Color,Oord16},
colors were quantized into discrete classes and treated as a multinomial distribution,
since generating images or predicting colors from grayscale images is usually a non-deterministic problem, 
\eg the color of a car can reasonably be red or white.
However, this convention is suboptimal for self-supervised learning of correspondences,
as we are not trying to generate colors for each pixel,
but rather, estimate a precise relocation of pixels in the reference frames.
More importantly,
quantizing the colors leads to an information loss that can be crucial for learning high-quality correspondences.

We conjecture that directly optimizing a regression loss between the reconstructed frame~($\hat{I_{t}}$) and real frame~($I_t$) will provide more discriminative training signals.
In this work, the objective $\mathcal{L}$ is defined as the Huber Loss:
\begin{align}
\mathcal{L} = \frac{1}{n} \sum_{i} z_{i}
\end{align}
\vspace{-.3cm}
\noindent where
\begin{align}
 z_{i} =
        \begin{cases}
        0.5 (\hat{\textbf{I}}^i_t - \textbf{I}^i_t)^2, & \text{if } |\hat{\textbf{I}}^i_t - \textbf{I}^i_t| < 1 \\
        |\hat{\textbf{I}}^i_t - \textbf{I}^i_t| - 0.5, & \text{otherwise }
        \end{cases}
\end{align}
where $\hat{\textbf{I}}^i_t$ refers to the pixel (a vector of $3$ values indicating RGB 
or Lab channels, normalized to the range [-1,1]) in the reconstructed frame that is copied from pixels in the reference frame~$I_{t-1}$,
and $I_t$ is the real frame at time point $t$.

% ------------------

\begin{figure*}[!htb]
  \centering
%  % Requires \usepackage{graphicx}
  \includegraphics[width=.95\textwidth]{figures/scheme_v10.pdf}
  \vspace{-3pt}
  \caption{Structure of MAST. 
  The current frame is used to compute \textbf{query} to attend and retrieve from memory (\textbf{key} \& \textbf{value}). 
  During training, we use raw video frame as \textbf{value} for self-supervision. 
  Once the encoder is trained, we use instance mask as \textbf{value}. See Section~\ref{sec:memory} for details.}
  \vspace{-5pt}
  \label{fig:scheme}
\end{figure*}
% ------------------

\vspace{5pt}
\subsection{Memory-augmented Tracking}
\label{sec:memory}
% {\color{red} Todo: transition}
So far we have discussed the straightforward attention-based mechanism for propagating
a mask from a single previous frame.
However, as predictions are made recursively,
errors caused by object occlusion and disocclusion tend to accumulate 
and eventually degrade the subsequent predictions.
To resolve this issue, we propose an attention-based tracker that \emph{efficiently} makes use of \emph{multiple} reference frames. 

\subsubsection{Multi-frame tracker}
An overview of our tracking model is shown in Figure~\ref{fig:scheme}.
To summarize the tracking process: given the current frame and multiple past frames (memory bank) as input,
we first compute the query Q from the current frame and a set of key (K), value (V) pairs from the memory frames.
Here we follow the general procedure in previous works as described in Sec.~\ref{sec:background},
where K and Q are computed from a shared-weight feature extractor and
V is equal to the input frame (during training) or object mask (during testing).
The computed affinity between Q and K is then used to make a prediction for each query pixel
based on V.

Note we don't put any weights on the frames,
as this should have been encoded in the affinity matrix, 
\emph{e.g.}~when the two frames are dis-similar due to temporal distance,
the corresponding similarity value will be naturally low,
and its label will have less contribution to the labeling of a target pixel.

The decision of which pixels to include in K is crucial for good performance.
Including all pixels previously seen is far too computationally expensive due to the quadratic explosion of the affinity matrix (\eg
the network of~\cite{Lai19} produces affinity matrices with more than 1 billion elements on 480p videos).
To reduce computation, \cite{Lai19} exploit temporal smoothness in videos
and apply restricted attention, only computing the affinity with pixels in a ROI around the query pixel location.
%The authors show that the method yields better performances and is computationally-efficient - \eg
%reducing size of similarity matrices by two orders of magnitude.
However, the temporal smoothness assumption holds only for temporally near frames.

To efficiently process temporally distant frames, we propose a two-step attention mechanism.
The first stage involves coarse pixel-matching with the frames in the memory bank to
determine ROIs that are likely to contain good matches with the query pixel.
In the second stage, we extract the ROIs and compute fine-grained pixel matching,
as described in Sec.~\ref{sec:background}.
Next, we describe the first coarse-matching stage in greater detail.
Overall, the process can be summarized in Algorithm~\ref{algorithm}.

\setlength{\textfloatsep}{2pt}% Remove \textfloatsep
\begin{algorithm}[!htb]
\small
  \caption{MAST} 
  \begin{algorithmic}[1]
    \State Choose $m$ reference frames $Q_1, Q_2, ... Q_m$
    \State Localize ROI $R_1, R_2, ... R_m$ according to 3.3.2 (Eq. 5 and 6) for each of the reference frames 
    \State Compute \textit{unnormalized} similarity matrix $A^{ij}_t = \langle\ R_t^i,K^j\rangle $  between target frame $K$ and each ROI.
    \State Normalize $A_{1..m}$ so that they altogether sum up to 1. 
    \State Output: pixel's label is determined by aggregating the labels of the ROI pixels (weighted by its affinity score).
  \end{algorithmic} 
\label{algorithm}
\end{algorithm}

%Next, the Query-Key-Value set is used to compute the current prediction with a simple  \textit{two-stage attention} process.
%In the first stage (\textit{ROI Localization}), for every  pixel in Query, we estimate a \textit{region of interest (ROIs)} in each Key. These ROIs represent a region where the  pixel in Query is likely to locate. For example, the football in Fig.~\ref{fig:scheme} to the right of the current frame should find the same football as ROIs in past frames.
% This process is explained in more detail in the section~\ref{sec:localization}.

%In the second stage, we compute a softmaxed similarity between these regions and the pixels in Query. This similarity is then used to retrieve Values from corresponding ROI regions as prediction. This second stage is a simple extension from the basic attention mechanism described in Sec.~\ref{sec:background}: we simply compute a \textit{single} softmax across space and time and sample only from ROIs.


% To resolve this challenge,
% we propose an attention-based model that can retrieve from multiple reference frames~
% (as shown in Figure~\ref{fig:scheme}). This
% allows longer-term correspondence matching for pixels occluded in the previous frame,
% but visible many frames earlier.
% However, this simple extension struggles for high-resolution dense tracking problems (or more generally computer vision problems),
% due to the quadratic explosion of the affinity matrix.
% For instance, when we use same network as~\cite{Lai19},
% the affinity matrix between two consecutive frames~(480p) exceeds dimension $30,000\times 30,000$.
% Processing multiple such affinity matrices is not only computationally unrealistic, but also unnecessary.

% To exploit temporal smoothness in videos,
% restricted attention~ \cite{Lai19} was applied,
% which effectively defines the candidate search region (in K) to be a local window around the query pixel.
% However,
% such restricted attention does not generalize to multiple reference frames further in time,
% as objects can move large distances or become occluded.

% In order to access and retrieve high-resolution information from the memory bank,
% we propose a deformable attention module that consists of ROI localization and fine-grained matching.
% In practice, a memory bank is composed of feature representations~(Keys) from multiple reference frames,
% \ie~$B = \{K_{t-1}, K_{t-2}, \cdots, K_1\}$.
% For each query pixel from the $t$-th frame, the goal is to coarsely filter frames in the memory bank,
% and pool out candidate regions from all reference frames to reconstruct the query pixel.
% =============
%\begin{figure}[!htb]
%  \centering
%  % Requires \usepackage{graphicx}
%  \includegraphics[width=.48\textwidth]{figures/self_attention_v1.pdf}
%  \vspace{-4pt}
%  \caption{Attention functions proposed in \cite{Lai19} and in this work. See text for details.}
%  \label{fig:self_attention}
%\end{figure}
% \vspace{-10pt}
% =============

\subsubsection{ROI Localization}
\label{sec:localization}
The goal of ROI localization is to estimate the candidate windows non-locally from memory banks. As shown in Figure~\ref{fig:ROI}, this can be achieved through restricted attention with varying dilation rate.

Intuitively, for short term memory (temporally close frames),
dilation is not required since spatial-temporal coherence naturally exists in videos;
%thus the $im2col$ falls back to the standard image-to-matrix transformation in ConvNets, 
thus ROI localization becomes restricted attention~(similar to \cite{Lai19}).
However, for long term memory (\eg the first frame),
we aim to account for the fact that objects can potentially appear anywhere in the reference frames.
We unify both scenarios into a single framework for learning ROI localization.
% ===============
\begin{figure}[H]
  \centering
%  % Requires \usepackage{graphicx}
  \includegraphics[width=.4\textwidth]{figures/NCF_v1.pdf}
  \vspace{-3pt}
  \caption{ROI Localization.}
  \label{fig:ROI}
\end{figure}
% ===============

Formally, for the query pixel $i$ in $I_t$ to localize the ROI from frame~($I_{t-N}$),
%the initial process can be described as:
we first compute $H^i_{t-N, x,y}$, the similarity heatmap between $i$ and all candidate pixels in the dilated window,
in parallel:
\begin{align}
H^i_{t-N, x,y} = softmax(Q^i_t \cdot im2col(K^i_{t-N}, \gamma_{t-N}))
\end{align}
where $\gamma_{t-N}$ refers to the dilation rate for window sampling in frame $I_{t-N}$ and $\gamma_{t-N} \propto N$,
and $im2col$ refers to an operation that transforms the input feature map into a matrix based on dilation rate. Specifically, in our experiments, we use $\gamma_{t-N} = \left \lceil (t-N)  / 15 \right \rceil$.

The center coordinates for ROIs can be then computed via a \textit{soft-argmax} operation:
\begin{align}
P^i_{x,y} = \sum_{x,y} H^i_{x,y} * C 
\end{align}
where $P_{xy}$ is the estimated center location of the candidate window in frame $I_{t-N}$ for query pixel $I^i_t$,
and $C$ refers to the grid coordinates~($x,y$) corresponding to the pixels in the window from $im2col$.
The resampled Key~($\hat{K}^i_{t-N}$) for pixel $I^i_t$ can be extracted with a bilinear sampler~\cite{Jaderberg2015}.
With all the candidate Keys dynamically sampled from different reference frames of the memory bank, 
each pixel can therefore emit the fine-grained matching with only these localized Keys,
resembling the standard restricted attention.
Therefore, with the proposed design, 
the memory-augmented model can efficiently access high-resolution information for correspondence matching, 
without incurring large physical memory costs.  

%\subsubsection{Why two-stage process}
%A basic solution for memory retrival is dot-product attention across all reference frames (Eq.~\ref{eq:attention} and \ref{eq:affinity}).
%However, this simple mechanism struggles for high-resolution tracking because of the quadratic explosion of the affinity matrix (\eg
%the network of~\cite{Lai19} produce affinity matrices with more than 1 billion elements on 480p videos).
%Although it allows memory retrival in theory, processing multiple such affinity matrices is simply computationally unrealistic.
%
%To exploit temporal smoothness in videos,
%\cite{Lai19} applies restricted attention,
%effectively placing the ROI around the query pixel.
%The authors show that the method yields better performances and is computationally-efficient - \eg
%reducing size of similarity matrices by two orders of magnitude.
%However,
%such restricted attention only works for close-by frames since large movement cannot be modelled.
%
%To get the best of both worlds, we borrow intuition from the classical coarse-to-fine process.
%The addition of ROI Localization module first coarsely filter frames in the memory bank, which is then processed for  fine-grained matching. By using the same window size, it models large movement without using any extra memory size compared to restricted attention.

% \subsubsection{Tracking from Multi-frames}
% {\color{red} Todo: add this section. explain technical details of making current prediction (\eg how to compute memory, multiple affinity matrix; how to warp multiple frames etc.). }


% \subsubsection{Matching \& Resampling}
% Once the ROIs are selected from multiple reference frames in the memory banks,
% the affinity matrix $A$ can be computed in a similar way to Eq.~\ref{eq:affinity},
% and the query pixel is reconstructed by a linear combination of all the pixels in the ROIs.
% Ideally, as objects can be occluded or disoccluded throughout the video,
% the query pixel will have a better chance of finding correspondences from the reference frames in the memory bank.


%we can use the pixel similarities to determine if the query pixel appears in the frame. 
%If a query pixel does not show up in a frame, the response in the ROI is all low. 
%In contrast, if a query pixel appear in a frame, 
%the response is high. 
%Since we aim to resample the query pixel from all memorized frames, 
%a simple solution is to find the weights to linearly combine the retrieved pixels and reconstruct the query pixel. 
%A natural solution is to find the weight is by applying a softmax acrossing both spatial and temporal dimension.

%\begin{align}
%A_{ijk} =  \frac{exp\langle\ f^i_t,f^j_k\rangle}{\sum_{jk} exp\langle\ f^i_t,f^j_{k}\rangle}
%\end{align}
%where $A$ stands for a similarity volume now.
%If the query pixel does not show up in some frames,
%the similarity of the entire frame is lower and the frame will be automatically ignored by the \textit{softmax} operation.

% \subsubsection{Bidirectional correspondence searching}
% When computing the reconstruction error, 
% the current methods only copy pixels from the previous frames.
% This can cause issues on pixels that are only visible in the curret frame, 
% but \emph{not visible} in any of the previous frames,
% Therefore, it violates the fundamental assumption that each pixel can be matched with pixels in previous frames,
% either introducing a high photometric loss or leading the model to compromise the matching performance, 
% and drift to other pixels in the neighborhood.
% These errors mainly come from two sources: pixels that are occluded or disoccluded, 
% and pixels at the boundary coming into the field of view.

% In fact, despite the time flows uni-directionally in the physical world, 
% there is no reason preventing us from exploring bidirectional correspondences in the videos.
% We can actually solve the aforementioned challenge by defining the loss as the minimum of bidrectional matching:
% \begin{align}
% L_p = min\{ L_{I_{t-1 \rightarrow t}},  L_{I_{t+1 \rightarrow t}} \}
% \end{align} 

%\subsection{Upperbound of Self-supervised Learning.}
%In order to demonstrate the power of self-supervised learning, 
%it is essential to train more powerful models.
%The model should at least be able to overfit the training set, 
%otherwise, we are not taking the core benefit of unsupervised learning.\\

%While checking the Table~3 in the BMVC paper,
%it is possible to outperform the supervised learning model with more diverse videos and models with higher capacity, \eg~ResNet-50, typical examples are.

%\subsection{Effectiveness of Finetuning on Dense Tracking.}
%\hl{Finetune the model with video segmentation masks, plot the relationships between the data for supervision and performance. }
%\vspace{0.5cm}

%\subsection{Instance Segmentation with the Self-supervised Representation}
%\hl{Take the learnt re. }
%\vspace{0.5cm}



% We propose a new attention function based on the restricted attention proposed , called \textit{deformable attention}. As shown in fig~\ref{fig:self_attention}, the new attention adds a component called \textit{ROI selection}, which estimate an offset from the given input. 


% Tracker drift remains a fundamental challenge for self-supervised dense tracking.
% As predictions are made recursively,
% errors caused by object occlusion and disocclusion tend to accumulate, 
% and eventually contaminate the subsequent predictions.
% In~\cite{Lai19},
% the authors proposed to alleviate the problem using scheduled sampling and forward-backward cycle consistency.

% In this section,
% we explore other possible solutions, \ie~augmenting the architecture with external memory modules.
% Specifically, we form a space-time non-local correspondence flow between the memory bank and the query image~(as shown in Figure~\ref{fig:scheme}). 
% Ideally, we want to enable each query pixel in the target frame to search all previous frames to find the optimal correspondence,
% however,
% this process is usually intractable as the memory required for computing the affinity matrix will grow quadratically.
% To strike a balance between computational cost and accuracy,
% %To obtain the offset value for each frame, 
% we take inspiration from pre-attentive processing,
% \ie information in previous video frames are coarsely processed to infer an offset for each query pixel, 
% and extract the regions with candidate reference pixels.
% These \emph{small regions} will therefore have the highest salience (a stimulus that stands out the most) or
% relevance to a query pixel, 
% and be bilinearly resampled from reference frames for attentive processing~(fine-grained correspondence matching).

% As an extension to the process described earlier~(Section~\ref{sec:background}),
% multiple reference frames from both long term~($I_{t-N}$, $N$ refers to the temporal gap)
% and short term memory~($I_{t-1}$) are fed as inputs to reconstruct the target frame~($I_t$).
% In the following sections,
% we describe the two core components that form the non-local correspondence flow:
% \textbf{ROI Localization} and \textbf{Matching \& Resampling}.

% %We then obtain all pixels in the query image by resampling from frames in the memory bank based on feature similarity. 
% %First, we estimate a rough region of interest (ROI), 
% %which is the most possible region that the query pixel resides in the corresponding frames. 
% %Next, instead of generating independent current frame prediction, 
% %we compute a single dot-product similarity volume between all ROIs and the query pixel. 
% %Finally, this volume is softmaxed and the query pixel is resampled as a linear combination
% %(weighted by aforementioned similarities) of pixels in all RoIs.  

% %\subsubsection{Non-local Correspondence Flow}
% %Figure~\ref{fig:Flow} illustrates the augmented correspondence flow, 
% %which is used to reconstruct the current frame with earlier frames. 
% %The non-local correspondence flow extends the correspondence flow with an offset, 
% %so that the representation could be used to model large movements. 
% %Taking two frames as input, ROI Localization first estimate the offset. 
% %A region of interest(ROI) is then extracted with a bilinear sampler at the offset location. 
% %Multiple such ROIs are extracted from several frames in the memory bank and used to match and resample the current pixel. 

% %
% % ===============
% %\begin{figure}[H]
% %  \centering
% %  % Requires \usepackage{graphicx}
% %  \includegraphics[width=.45\textwidth]{figures/flow_v1.pdf}
% %  \vspace{-3pt}
% %  \caption{Non-local Correspondence Flow. See text for details. }
% %  \label{fig:Flow}
% %\end{figure}
% % ===============



==> sec/teaser.tex <==
% %!TEX root=../egpaper_for_review.tex


% \begin{table}[htbp]
% \centering
% \small
% \begin{tabular}{cccccc}
% \hline
% Methods    & Arch    & Supervised      & Dataset       & Speed     & J\& F        \\ \hline
% Methods    & Arch    & Supervised      & Dataset       & Speed     & J\& F

% \end{tabular}
% \caption{To be filled in.}\label{table:teaser}
% \end{table}

==> tables/ablation_0.tex <==
%!TEX root=../egpaper_for_review.tex
\begin{table*}
\centering
% \footnotesize
\footnotesize\addtolength{\tabcolsep}{-1pt}
\begin{minipage}{.3\textwidth}
\centering

\begin{tabular}{ccc}

        \toprule
        I-F Align  & $\mathcal{J}$(Mean)  & $\mathcal{F}$(Mean)   \\ \midrule

        No        & 59.1  & 64.0        \\
        Yes       & \textbf{61.2}  & \textbf{66.3}      \\ 
        \midrule
         & $+2.1$ & $+2.3$  \\
        \bottomrule

\end{tabular}
\caption{Effect of training colorspaces on dense tracking. Plus sign denote multiple training signals. Higher values are better. }

\end{minipage} \hfill
\begin{minipage}{.35\textwidth}
\centering

    \begin{tabular}{cccc}

        \toprule
        Memory  & agg. & $\mathcal{J}$(Mean)  & $\mathcal{F}$(Mean)   \\ \midrule


        Only long 	&  \xmark  & 				   \\
        \midrule
        Only short  &  \xmark  &  &   \\
        % Only short term    &  \cmark    & 57.3 & 61.8   \\
        \midrule
        Both    &  ave  & -  & -      \\
        Both    &  max  & \textbf{61.2}  & \textbf{66.3} \\
        Both    &  ST  & \textbf{61.2}  & \textbf{66.3}    
              \\ 
        \bottomrule

    \end{tabular}
    \caption{Effect of training colorspaces on dense tracking. Plus sign denote multiple training signals. Higher values are better. }

\end{minipage}
\begin{minipage}{.3\textwidth}
\centering

\begin{tabular}{ccc}

        \toprule
        Propagation  & $\mathcal{J}$(Mean)  & $\mathcal{F}$(Mean)   \\ \midrule

        Soft        & 59.1  & 64.0        \\
        Hard       & \textbf{61.2}  & \textbf{66.3}      \\ 
        \midrule
         & $+2.1$ & $+2.3$  \\
        \bottomrule

\end{tabular}
\caption{\textbf{Propagating soft prob. \textit{vs.} hard max}: Effect of training colorspaces on dense tracking. Plus sign denote multiple training signals. Higher values are better. }

\end{minipage} \hfill
\begin{minipage}{.6\textwidth}
\centering

\begin{tabular}{cccccc}

\toprule
Colors.  & Loss & $\mathcal{J}$(Mean)  & $\mathcal{J}$(Recall) & $\mathcal{F}$(Mean)  & $\mathcal{F}$(Recall) \\
\midrule
\multirow{2}{*}{RGB}   &  Cls.  & 52.7  & 57.1       \\
   &  Reg.  & 52.7  & 57.1       \\
\midrule

 \multirow{2}{*}{HSV} &  Cls.    & 54.3 & 58.6  \\
  &  Reg.    & 54.3 & 58.6  \\

\midrule

\multirow{2}{*}{Lab}  &  Cls.   & \textbf{61.2}  & \textbf{66.3}\\ 
 &  Reg.  & \textbf{61.2}  & \textbf{66.3}\\ 

\bottomrule

\end{tabular}
\caption{\textbf{Training colorspaces and loss}: Our final model trained with Lab colorspace with regression loss outperforms all other models on dense tracking task. Higher values are better. }

\end{minipage} \hfill
\begin{minipage}{.3\textwidth}
\centering

\begin{tabular}{cccc}
\toprule
Input  &  Loss & $\mathcal{J}$(Mean)  & $\mathcal{F}$(Mean) \\
\midrule
Lab   & RGB     & \textbf{61.2}  & \textbf{66.3}       \\ 
RGB   & Lab     & \textbf{61.2}  & \textbf{66.3}       \\ 
\midrule
Lab   & Lab     & \textbf{61.2}  & \textbf{66.3}       \\ 
        % Lab+HSV    & todo & todo                     \\
        % Lab+HSV+RGB & todo & todo                     \\

        \bottomrule

\end{tabular}
\caption{\textbf{Cross color space matching \textit{vs.} single color space}: Effect of training colorspaces on dense tracking. Plus sign denote multiple training signals. Higher values are better. }

\end{minipage} \hfill
% \begin{minipage}{.35\textwidth}
% \centering

%     \begin{tabular}{ccc}
%     \toprule
%     Dataset  & $\mathcal{J}$(Mean)  & $\mathcal{F}$(Mean)  \\ 
%     \midrule

%     VID         & 60.0 & 63.9    \\ 
%     Kinetics    & todo & todo           \\
%     OxUvA       & 61.2  & 66.3    \\

%     \bottomrule
%     \end{tabular}
%     \caption{Effect of training colorspaces on dense tracking. Plus sign denote multiple training signals. Higher values are better. }

% \end{minipage}
\end{table*}



==> tables/color.tex <==
%!TEX root=../egpaper_for_review.tex

% ===============
\begin{table}[h]
\centering
\footnotesize\addtolength{\tabcolsep}{-5pt}
\begin{tabular}{c @{\extracolsep{\fill}} ccccc}
\toprule
Colorspace  & $\mathcal{J}$(Mean)  & $\mathcal{F}$(Mean) &  \\ \midrule

Lab        & 61.2  & 66.3       \\ 
RGB        & 52.7  & 57.1       \\
HSV        & 54.3 & 58.6                     \\
% Lab+HSV    & todo & todo                     \\
% Lab+HSV+RGB & todo & todo                     \\
  
\bottomrule
\end{tabular}
\vspace{-8pt}
\caption{Effect of training colorspaces on dense tracking. Plus sign denote multiple training signals. Higher values are better. }
\label{table:color_1}
\end{table}


==> untitled folder/def.tex <==
\newcommand{\TODO}[1]{\textcolor{red}{#1}}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\norm}[1]{\left\lVert #1 \right\rVert}
\newcommand{\matr}[1]{\mathbf{#1}}

\newcommand{\reals}[1]{\mathbb{R}^{#1}}
\newcommand{\set}[1]{\left\{{#1}\right\}}
\newcommand{\transpose}[1]{#1^\top}
\newcommand*\rot{\rotatebox{90}}

\newcommand{\seqset}{\mathcal{S}}
\newcommand{\enorm}[1]{\left\|{#1}\right\|_2}
\DeclareMathOperator{\loss}{loss}
\newcommand{\binary}[1]{\mathbb{B}^{#1}}
\newcommand{\one}{\mathbf{1}}
\newcommand{\comment}[1]{}

\usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%



==> untitled folder/sec/exp.tex <==
%!TEX root=../egpaper_for_review.tex
\section{Experiments}
\label{sec:experiments}
% ===============
\input{./tables/davis-2017.tex}
We benchmark our model on two public benchmarks:
DAVIS-2017~\cite{Pont-Tuset17}  and the current largest video segmentation dataset, YouTube-VOS~\cite{Xu18}.
The former contains 150 HD videos with over 30K manual instance segmentations,
and the latter has over 4000 HD videos of 90 semantic categories, totalling over 190k instance segmentations.
For both datasets,
we benchmark the proposed self-supervised learning architecture~(MAST) on the official semi-supervised video segmentation setting~(\emph{aka.}~dense tracking),
where a ground truth instance segmentation mask is given for the first frame, 
and the objective is to propagate the mask to subsequent frames.
In Section~\ref{sec:davis},  
we report performance of our full model and several ablated models on the DAVIS benchmark.
Next, in Section~\ref{sec:youtube_vos}, we analyze the \emph{generalizability} of our model by benchmarking on the large-scale YouTube-VOS dataset.

% --------------------
\begin{figure*}[!htb]
  \centering
  \includegraphics[width=\textwidth]{figures/qualitative_with_others_v2.pdf}
  \vspace{-10pt}
  \caption{Our method vs. previous self-supervised methods. 
  Other methods show systematic errors in handling occlusions. Row 1: The dancer undergoes large self-occlusion. 
  %, causing other methods to lose track (TC and CF) or over segment (OSVOS).
  Row 2: The dog is repeatedly occluded by poles. 
  %, and other methods show different degrees of loss in track (especially VC and TC).
  Row 3: Three women reappear after being occluded by the man in the foreground.
  % Three other propagation-based methods without memory-augmentation (VC,TC,CF) fail severely.
  }
    \vspace{-1.5em}
  \label{fig:qualitative_2}
\end{figure*}
%
\vspace{3pt}
\par \noindent \textbf{Standard evaluation metrics.} 
We use region similarity~($\mathcal{J}$) and contour accuracy~($\mathcal{F}$) to evaluate the tracked instance masks~\cite{Perazzi16}.

\vspace{3pt}
\par \noindent \textbf{Generalizability metrics} 
To demonstrate the generalizability of tracking algorithms in category-agnostic scenarios,
\ie~the categories in training set and testing set are disjoint,
YouTube-VOS also explicitly benchmarks the performances on unseen categories.
We therefore evaluate a \emph{generalization gap} in Section~\ref{sec:gen}, 
which is defined as the average performance difference between seen and unseen object classes:
\begin{align}
\text{Gen. Gap} = \frac{(\mathcal{J}_{seen} - \mathcal{J}_{unseen}) + (\mathcal{F}_{seen}  - \mathcal{F}_{unseen})}{2}
\end{align}
Note, the proposed metric aims to explicitly penalize the case where the performance on seen outperforms unseen by large margins,
while at the same time provide a reward when the performance on unseen categories is higher than on seen ones.

% ---------------
\subsection{Video Segmentation on DAVIS-2017}
\label{sec:davis}
\subsubsection{Main results}
% ---------------
In Table~\ref{table:davis_1}, 
we compare MAST with previous approaches on the DAVIS-2017 benchmark. 
Two phenomena can be observed:
\emph{first},
our proposed model clearly outperforms all other self-supervised methods,
surpassing previous state-of-the-art CorrFlow by a significant margin~($65.5$ vs $50.3$ on $\mathcal{J}$\&$\mathcal{F}$).
\emph{Second}, 
despite using only ResNet18 as the feature encoder,
our model trained with self-supervised learning can still surpass supervised approaches that use heavier architectures.
% --------------------

% ===============
\vspace{-10pt}
\subsubsection{Ablation Studies}
\label{exp:ablation}
To examine the effects of different components, 
we conduct a series of ablation studies by removing one component at a time.
All models are trained on OxUvA~(except for the analysis on different datasets), 
and evaluated on DAVIS-2017 semi-supervised video segmentation~(\emph{aka.}~dense tracking) \emph{without} any finetuning.\\[-8pt]
% ===============
\input{tables/ablation.tex}
% ===============
% --------------------
\par \noindent  \textbf{Choice of color spaces.}
% --------------------
As shown in Table~\ref{tab:abl_color}, 
we perform different experiments with input frames transformed into different color spaces, \eg~RGB, $Lab$ or HSV.
We find that the MAST model trained with $Lab$ color space always outperforms the other color spaces,
validating our conjecture that dropout in a decorrelated color space leads to better feature representations for self-supervised dense tracking, as explained in Section~\ref{sec:color}.
Additionally, 
we compare our default setting with a model trained with cross-color space matching task~(shown in Table~\ref{tab:abl_cross_color}).
That means to use a different color space for the input and the training objective, 
\eg~input frames are in RGB, and loss function is defined in $Lab$ color space.
Interestingly, the performance drops significantly, 
we hypothesis this can attribute to the fact that all RGB channels include a representation of brightness,
making it highly correlate to the luminance in $Lab$, 
therefore acting as a weak information bottleneck.\\[-8pt]
% % --------------------
\par \noindent  \textbf{Loss functions.}
% % --------------------
As a variation of our training procedure, 
we experiment with different loss functions: 
cross entropy loss on the quantized colors, and photometric loss with Huber loss.
As shown in Table~\ref{tab:abl_color}, 
regression with real-valued photometric loss surpasses classification significantly,
validating our conjecture that the information loss during color quantization results in inferior representations for self-supervised tracking~(as explained in Section~\ref{sec:training_signal}),
due to less discriminative training signals.\\[-8pt]
% --------------------
\par \noindent  \textbf{Image feature alignment.}
% --------------------
To evaluate the alignment module proposed for aligning features with the original image, 
we compare it to direct bilinear image downsampling used by CorrFlow~\cite{Lai19}. 
The result in Table~\ref{tab:abl_align} shows that our approach achieves about $2.2\%$ higher performance.\\[-8pt]

% --------------------
\par \noindent  \textbf{Dynamic memory by exploiting more frames.}
% --------------------
% {\color{red} TODO: make this clear}
We compare our default network with variants that have only short term memory or long term memory. 
Results are shown in Table~\ref{tab:abl_mem}.
While both short term memory and long term memory alone can make reasonable predictions,
the combined model achieves the highest performance.
The qualitative predictions~(Figures~\ref{fig:qualitative} and~\ref{fig:qualitative_2}) also confirm that the improvements come from reduced tracker drift.
For instance, when severe occlusion occurs, 
our model is able to attend and retrieve high-resolution information from frames that are temporally distant. 
%As shown in Figure~\ref{fig:mem_perf}, we explicitly evaluate the effectiveness of using multiple reference frames,
%specifically, when only the first frame is stored in the memory, 
%the $\mathcal{J} \& \mathcal{F}$ is only around $46$,
%the number of frames 
%we confirm that a 5-frame memory is optimal for our task.

% ===============
%\begin{figure}[H]
%  \centering
%  \includegraphics[width=.45\textwidth]{figures/fig_mem_v1.pdf}
%  \vspace{-2pt}
%  \caption{\textbf{Optimal memory size}: 
%  The performance of our model first increases when number of frame in memory grows. After memory reaches 5 frames, the performance plateaued. }
%  \label{fig:mem_perf}
%\end{figure}
% ===============
% hypothesize that since the tracked objects may often be occluded or deformed,
%it is unreasonable to force each ROI to share importance.
%Aggregating similarity across the temporal dimension alleviates the issue:
%ROIs that have low overall similarity are ignored by a global softmax operation.  
% \\[-5pt]
% --------------------
%\paragraph{Soft vs. Hard mask propagation}
% --------------------
%As shown in Table~\ref{tab:abl_prop}, 
%we show the soft mask propagation is beneficial.
% --------------------
% \par \noindent  \textbf{Choice of training data.}
% % --------------------
% As shown in Table~\ref{tab:abl_dataset}, 
% we train SMAT on different datasets: 
% ImageNet VID~\cite{Deng09}, OxUvA~\cite{Valmadre18}, and YouTube-VOS~\cite{Xu18} training splits.
% The model trained on ImageNet VID shows slightly worse performance on the dense tracking task,
% which we conjecture is because the dataset contains relatively short videos, 
% therefore fewer challenging scenarios that lead to tracker drift will appear, \eg~occlusion or disocclusion.
% Despite the small variation in performance, 
% the results still show that the proposed architecture and training scheme are generally successful and
% not due to well-selected training data.
% % ===============

\subsection{Youtube Video Object Segmentation}
\label{sec:youtube_vos}
We also evaluate the MAST model on the Youtube-VOS validation split~(474 videos with 91 object categories).
As no other self-supervised methods have been tested on the benchmark, 
we directly compare our results with supervised methods. 
As shown in Table~\ref{table:youtube_1}, 
our method outperforms the other self-supervised learning approaches by a significant margin~($64.2$ vs.~$46.6$), 
and even achieves comparable performance to many heavily supervised methods. 

% ===============
\input{tables/youtube-vos.tex}
% ===============
\subsubsection{Generalizability}
\label{sec:gen}
As another metric for evaluating category-agonostic tracking, 
the YouTube-VOS dataset conveniently has separate measures for seen and unseen object categories. 
We can therefore estimate testing performance on out-of-distribution samples to gauge the model's generalizability to more challenging, unseen, real-world scenarios. 
As seen from the last two columns, we rank second amongst all algorithms in unseen objects. 
In these unseen classes, 
we are even $3.9\%$ higher than the DAVIS 2018 and YouTube-VOS 2018 video segmentation challenge winner, 
PreMVOS\cite{Luiten18}, 
a complex algorithm trained with multiple large manually labeled datasets.
For fair comparison, 
we train our model only on the YouTube-VOS training set. We also re-train two most relevant self-supervised methods in the same manner as baselines. % (so the `Seen' and `Unseen' separation holds true to our model). 
Even learning from only a subset of all classes, 
our model generalizes well to unseen classes,
with a generalization gap (\ie the performance difference between seen and unseen objects) near zero ($0.4$). 
This gap is much smaller than any of the baselines ($\text{avg}=11.5$), 
suggesting a unique advantage to most other algorithms trained with labels. 

By training on large amounts of unlabeled videos, 
we learn an effective tracking representation without the need for any human annotations. 
This means that the learned network is not limited to a specific set of object categories (\ie those in the training set),
but is more likely to be a ``universal feature representation'' for tracking.
Indeed, the only supervised algorithm that is comparable to our method in generalizability is OSVOS (2.7 \textit{vs.} 0.4). 
However, OSVOS uses the first image from the testing sequence to perform costly domain adaptation, \eg~one-shot fine-tuning. 
In contrast, our algorithm requires no fine-tuning, which further demonstrates its zero-shot generalization capability. 

Note our model also has a smaller generalization gap compared to other self-supervised methods as well. 
This further attests to the robustness of its learned features, 
suggesting that our improved reconstruction objective is highly effective in capturing general features. 

%This could suggest that our model learns more class-agnostic features - making it another valuable aspect of our method.

==> untitled folder/sec/exp_v0.tex <==
%!TEX root=../egpaper_for_review.tex
\section{Experiments}
% As a fair comparison, 
% we pursue minimal changes made to the baseline systems~\cite{Lai19}, 
% and pinpoint the keys to build dense tracking systems purely based on self-supervised learning from videos.
% ===============
\input{./tables/davis-2017.tex}
We benchmark our model on two public benchmarks:
DAVIS-2017~\cite{Pont-Tuset17}  and the current largest video segmentation dataset, YouTube-VOS~\cite{Xu18}.
For both datasets,
a ground truth instance segmentation mask is given for the first frame, 
and the objective is to propagate the mask to subsequent frames.
In Section~\ref{sec:davis},  
we report performance of our full model and several ablated models on DAVIS benchmark.
Next, in Section~\ref{sec:youtube_vos}, we analyze the \emph{generalizability} of our model by benchmarking on the large-scale YouTube-VOS dataset.

\vspace{3pt}
\par \noindent \textbf{Standard evaluation metrics.} 
We use region similarity~($\mathcal{J}$) and contour accuracy~($\mathcal{F}$) to evaluate the tracked instance masks~\cite{Perazzi16}.

\vspace{3pt}
\par \noindent \textbf{Generalizability metrics} 
In order to demonstrate the generalizability of tracking algorithms under category-agnostic scenarios,
\ie~the categories in training set and testing set are disjoint,
YouTube-VOS also explicitly benchmarks the performances on unseen categories.
We therefore evaluate a generalization gap in Section~\ref{sec:gen}, 
which is defined as the average performance difference between seen and unseen object classes:
\begin{align}
\text{Gen. Gap} = \frac{(\mathcal{J}_{seen} - \mathcal{J}_{unseen}) + (\mathcal{F}_{seen}  - \mathcal{F}_{unseen})}{2}
\end{align}

% ---------------
\subsection{Video Segmentation on DAVIS-2017}
\label{sec:davis}
\subsubsection{Main results}
% ---------------
In Table~\ref{table:davis_1}, 
we compare MAST with previous approaches on the DAVIS-2017 benchmark. 
Two phenomena can be observed:
\emph{first},
our proposed model has clearly dominated all the other self-supervised methods,
surpassing previous state-of-the-art CorrFlow by a significant margin~($65.5$ vs $50.3$ on $\mathcal{J}$\&$\mathcal{F}$).
\emph{Second}, 
despite only using ResNet18 as feature encoder,
our model trained with self-supervised learning can still surpass some of the results by heavily supervised learning.

% \subsubsection{Qualitative Results}
% % ===============
% As shown in Figure~\ref{fig:qualitative} and Figure~\ref{fig:qualitative_2}, 
% SMAT can propagate the segmentation mask through sequences even in the presence of large scale variation from camera motion, 
% and large object deformation. 

% --------------------
\begin{figure*}[!htb]
  \centering
%  % Requires \usepackage{graphicx}
  \includegraphics[width=\textwidth]{figures/qualitative_with_others_v2.pdf}
  \vspace{-3pt}
  \caption{Our method vs. previous self-supervised methods. 
  Other methods show systematic errors in handling occlusions. Row 1: The dancer undergoes large self-occlusion. %, causing other methods to lose track (TC and CF) or over segment (OSVOS).
  Row 2: The dog is repeatedly occluded by poles. %, and other methods show different degrees of loss in track (especially VC and TC).
  Row 3: Three women reappear after being occluded by the man in the foreground.% Three other propagation-based methods without memory-augmentation (VC,TC,CF) fail severely.
  }
    \vspace{-1.5em}

  \label{fig:qualitative_2}
\end{figure*}
%
% --------------------

% ===============
\vspace{-5pt}
\subsubsection{Ablation Studies}
\label{exp:ablation}

To examine the effects of different components, 
we conduct a series of ablation studies by removing one component at a time.
All models are trained on OxUvA~(except the analysis on dataset), 
and evaluated on the dense tracking task~(semi-supervised video segmentation on DAVIS-2017) \emph{without} any finetuning.  
\\[-5pt]
% ===============
\input{tables/ablation.tex}
% ===============
% --------------------
\par \noindent  \textbf{Choice of color spaces.}
% --------------------
As shown in Table~\ref{tab:abl_color}, 
we perform different experiments with input frames transformed into different color spaces, \eg~RGB, $Lab$ or HSV.
We find that the MAST model trained with $Lab$ color space always outperforms the other color spaces,
validating our conjecture that dropout in a decorrelated color space leads to better feature representations for self-supervised dense tracking, as explained in Section~\ref{sec:color}.
Additionally, 
we compare our default setting with a model trained with cross-color space matching task~(shown in Table~\ref{tab:abl_cross_color}).
That means to use a different color space for the input and the training objective, 
\eg~input frames are in RGB, and loss function is defined in $Lab$ color space.
Interestingly, the performance drops significantly, 
we hypothesis this can attribute to the fact that all RGB channels include a representation of brightness,
making it highly correlate to the luminance in $Lab$, 
therefore acting as a weak information bottleneck.
\\[-10pt]
% % --------------------
\par \noindent  \textbf{Loss functions.}
% % --------------------
As a variation of our training procedure, 
we experiment with different loss functions: 
cross entropy loss on the quantized colors, and photometric loss with Huber loss.
As shown in Table~\ref{tab:abl_color}, 
regression with real-valued photometric loss surpasses classification significantly,
validating our conjecture that the information loss during color quantization ends up with inferior representations for self-supervised tracking~(as explained in Section~\ref{sec:training_signal}),
due to less discriminative training signals.
\\[-5pt]
% --------------------
\par \noindent  \textbf{Image feature alignment.}
% --------------------
To evaluate the alignment module proposed for aligning features with the original image, 
we compare it to direct bilinear image downsampling used by CorrFlow\cite{Lai19}. 
The result in Table~\ref{tab:abl_align} shows that our approach achieves about $2.2\%$ higher performance.  
\\[-5pt]

% --------------------
\par \noindent  \textbf{Dynamic memory by exploiting more frames.}
% --------------------
% {\color{red} TODO: make this clear}
We compare our default network with variants that have only short term memory or long term memory. 
Results are shown in Table~\ref{tab:abl_mem}.
While both short term memory and long term memory alone can make reasonable predictions,
the combined model achieves the highest performance.
The qualitative predictions~(Figures~\ref{fig:qualitative} and~\ref{fig:qualitative_2}) also confirm that the improvements come from reduced tracker drift.
For instance, when severe occlusion occurs, 
our model is able to attend and retrieve high-resolution information from frames that are temporally distant. In Fig.~\ref{fig:mem_perf}, we confirm that a 5-frame memory is optimal for our task.

% ===============
\begin{figure}[H]
  \centering
  \includegraphics[width=.45\textwidth]{figures/fig_mem_v1.pdf}
  \vspace{-2pt}
  \caption{\textbf{Optimal memory size}: 
  The performance of our model first increases when number of frame in memory grows. After memory reaches 5 frames, the performance plateaued. }
  \label{fig:mem_perf}
\end{figure}
% ===============
% hypothesize that since the tracked objects may often be occluded or deformed,
%it is unreasonable to force each ROI to share importance.
%Aggregating similarity across the temporal dimension alleviates the issue:
%ROIs that have low overall similarity are ignored by a global softmax operation.  
% \\[-5pt]
% --------------------
%\paragraph{Soft vs. Hard mask propagation}
% --------------------
%As shown in Table~\ref{tab:abl_prop}, 
%we show the soft mask propagation is beneficial.
% --------------------
% \par \noindent  \textbf{Choice of training data.}
% % --------------------
% As shown in Table~\ref{tab:abl_dataset}, 
% we train SMAT on different datasets: 
% ImageNet VID~\cite{Deng09}, OxUvA~\cite{Valmadre18}, and YouTube-VOS~\cite{Xu18} training splits.
% The model trained on ImageNet VID shows slightly worse performance on the dense tracking task,
% which we conjecture is because the dataset contains relatively short videos, 
% therefore fewer challenging scenarios that lead to tracker drift will appear, \eg~occlusion or disocclusion.
% Despite the small variation in performance, 
% the results still show that the proposed architecture and training scheme are generally successful and
% not due to well-selected training data.
% % ===============

\subsection{Youtube Video Object Segmentation}
\label{sec:youtube_vos}
We also evaluate the MAST model on the Youtube-VOS validation split~(474 videos with 91 object categories).
As no other self-supervised methods have been tested on the benchmark, 
we directly compare our results with supervised methods. 
As shown in Table~\ref{table:youtube_1}, 
our method achieves results comparable to many heavily supervised methods. 

% ===============
\input{tables/youtube-vos.tex}
% ===============
\subsubsection{Generalizability}
\label{sec:gen}
As another metric for evaluating category-agonostic tracking, 
the YouTube-VOS dataset has conveniently separate measures for seen and unseen object categories. 
We can therefore estimate testing performance on out-of-distribution samples to gauge the model's generalizability to more challenging, unseen, real-world scenarios. 
As seen from the last two columns, we rank second amongst all algorithms in unseen objects. 
In these unseen classes, 
we are even $3.9\%$ higher than the DAVIS 2018 and YouTube-VOS 2018 video segmentation challenge winner, 
PreMVOS\cite{Luiten18}, 
a complex algorithm trained with multiple large manually labeled datasets.
For fair comparison, 
we train our model only on the YouTube-VOS training set. We also re-train two most related self-supervised methods in the same manner as baselines. % (so the `Seen' and `Unseen' separation holds true to our model). 
Even learning from only a subset of all classes, 
our model generalizes well to unseen classes,
with a generalization gap (\ie the performance difference between seen and unseen objects) near zero ($0.4$). 
This gap is much smaller than any of the baselines ($\text{avg}=11.5$), 
suggesting a unique advantage to most other algorithms trained with labels. 

By training on large amount of unclassified videos, the feature extractor is learned without using any information of object classes. This means that the learned feature is more independent to a specific set of object class (\ie those in the training set). Therefore, the process is more close to an optimal ``universal feature extraction'', \ie features should contain less manual and hand-crafted information. Indeed, the only supervised algorithm that is comparable to our method in generalizability is OSVOS (2.7 \textit{vs.} 0.4). However, OSVOS uses the first image from the testing sequence to perform a costly one-shot fine-tuning. This is inferior to our algorithm, which has zero-shot generalization ability. 

Note our model also has a smaller generalization gap compared to other self-supervised methods as well. This further attesting to the robustness of its learned features, suggesting that our improved reconstruction objective is highly effective in capturing general features. 

%This could suggest that our model learns more class-agnostic features - making it another valuable aspect of our method.

==> untitled folder/sec/imp.tex <==
%!TEX root=../egpaper_for_review.tex
\section{Implementation Details}
\noindent\textbf{Training: }
For fair comparison,
we adopt as our feature encoder the same architecture~(ResNet18) as~\cite{Lai19} in all experiments~(as shown in Supplementary Material).
The network produces feature embeddings with a spatial resolution $1/4$ of the original image.
The model is trained in a completely self-supervised manner,
meaning the model is initialized with random weights, 
and we do \emph{not} use any information other than raw video sequences.
We report main results on two training datasets: OxUvA~\cite{Valmadre18} and YouTube-VOS (both raw videos only). 
We report the first for fair comparison with the state-of-the-art method~\cite{Lai19} and the second for maximum performance. 
As pre-processing, we resize all frames to $256\times 256\times3$. 
In all of our experiments, 
we use $I_0$,  $I_5$~(only if the index for the current frame is larger than $5$) as long term memory, 
and {$I_{t-5}$, $I_{t-3}$, $I_{t-1}$} as short term memory. 
Empirically, we find the choice of frame number has small impact on performance, 
but using both long and short term memory is essential~(See appendix). \\[3pt]
%
During training, 
we first pretrain the network with a pair of input frames, 
\ie~one reference frame and one target frame are fed as inputs.
One of the color channels is randomly dropped with probability $p=0.5$.
We train our model end-to-end using a batch size of $24$ for 1M iterations with the Adam optimizer. 
The initial learning rate is set to $1e$-3, and halved after 0.4M, 0.6M and 0.8M iterations. 
We then finetune the model using multiple reference frames (our full memory-augmented model) 
with a small learning rate of $2e$-5 for another 1M iterations.
As discussed in Section~\ref{sec:loss}, 
the model is trained with a photometric loss between the reconstruction and the true frame. \\[3pt]
%
\noindent\textbf{Inference: }
We use the trained feature encoder to compute the
affinity matrix between pixels in the target frame and those in the reference frames. 
The affinity matrix is then used to propagate the desired pixel-level entities,
such as instance masks in the dense tracking case, 
as described in Algorithm~\ref{algorithm}.  \\[3pt]
%
\noindent\textbf{Image Feature Alignment: }
Due to memory constraints, 
the supervision signals in previous methods were all defined on bilinearly downsampled images.
As shown in Figure~\ref{fig:align}(a), this introduces a misalignment between strided convolution layers 
and images from na\"ive bilinear downsampling. 
We handle this spatial misalignment between feature embedding and image by directly sampling at the strided convolution centers.
This seemingly minor change actually brings significant improvement to the downstream tracking task (Table~\ref{tab:abl_align}).
% ===============
\begin{figure}[t]
  \centering
%  % Requires \usepackage{graphicx}
  \includegraphics[width=.48\textwidth]{figures/sampling_v3.pdf}
  \vspace{-15pt}
  \caption{Image Feature Alignment. We fix the misalignment between strided convolution layers (with kernel centered at red circle) and images from na\"ive bilinear downsampling (with kernel centered at blue dot) by sampling directly at the strided convolution centers.}
  \label{fig:align}
\end{figure}
% ===============

% The key idea is to maintain a memory bank~(sample frames from previous time point),
% in order to reconstruct frame $I_t$, 
% we compute the affinity matrix with $I_{t-1}$, $M_1, \dots M_k$~(assume we maintain $k$ frames as in the memory), 
% and then compute the reconstructed frames for $t$ time points by copying from all these memory banks, 
% getting predictions $\hat{I}_{I_{t-1} \rightarrow I_t}$, $\hat{I}_{I_{M_1} \rightarrow I_t}$, $\dots$, $\hat{I}_{I_{M_k} \rightarrow I_t}$.
% The loss function for backpropagation is therefore defined as,
% \begin{align}
% J = \sum_i min( L(I_t, \hat{I}_{I_{t-1} \rightarrow I_t}), L(I_t, \hat{I}_{I_{M_1} \rightarrow I_t}), \dots, L(I_t, \hat{I}_{I_{M_k} \rightarrow I_t}))
% \end{align}
% $i$ refers to the pixels over the entire image.



==> untitled folder/sec/intro.tex <==
%!TEX root=../egpaper_for_review.tex

Although the working mechanisms of human visual system remain somewhat obscure at the level of neurophysiology, 
it is a general concensus that tracking objects is a fundamental ability that a baby starts developing since two to three months age~\cite{Brazelton66, Kremenitzer79, Hofsten82}. 
Similarly, in computer vision systems, 
tracking plays key roles in a large number of applications ranging from autonomous driving to video surveillance. 

% =========================
\begin{figure}[t]
\includegraphics[width=0.5\textwidth]{figures/fig1.pdf}
\centering
\vspace{-0.5cm}
\caption{Comparison with other recent works on the DAVIS-2017 benchmark, 
\ie dense tracking or instance-wise video segmentation given the first frame annotation.
The proposed dense tracking system achieves state-of-the-art performance among all self-supervised approaches,
even comparable to some approaches trained with heavy supervision with ImageNet, COCO, Pascal, DAVIS, Youtube-VOS.\\
\textbf{Notation}:
CorrFlow~\cite{Lai19}, CycleTime~\cite{Wang19}, mgPFF~\cite{Song19}, Colorization~\cite{Vondrick18},
OSVOS~\cite{Caelles17}, VideoMatch~\cite{Hu18}, RGMP~\cite{Oh18}, OnAVOS~\cite{Voigtlaender17}, 
OSMN~\cite{Yang18}, FAVOS~\cite{Cheng18}, OSVOS-S~\cite{Maninis18}, FEELVOS~\cite{Voigtlaender19}, 
DyeNet~\cite{Li18ECCV}, PReMVOS~\cite{Luiten18}.}
\label{fig:teaser}
\vspace{-10pt}
\end{figure}
% =========================

Given arbitrary objects defined in the first frame, 
a tracking algorithm aims to relocate the same object throughout the entire video sequence. 
In the literature, 
tracking can be cast into two categories:
One is typically termed Visual Object Tracking (VOT)~\cite{VOT_TPAMI}, 
the goal is to relocalize the objects with bounding boxes through the video;
The other one aims for more fine-grained tracking, \ie relocalize the objects with segmentation masks,
this is recently put in the name of Semi-supervised Video Object Segmentation (Semi-VOS)~\cite{Pont-Tuset17}.
In this paper, we focus on the latter case. 
To avoid abuse of terminology, this is termed as \emph{dense Tracking} from here on. 

% ===============
\begin{figure*}[!htb]
  \centering
%  % Requires \usepackage{graphicx}
  \includegraphics[width=.98\textwidth]{figures/qualitative_v3.pdf}
  \vspace{-3pt}
  \caption{Qualitative results from our \emph{self-supervised dense tracking model} on DAVIS-2017 and YouTube-VOS dataset. 
 The number on top left refers to the frame number in the video.
 For all examples, the mask for $0th$ frame is given, and the task is to track the objects along the video.
 Our self-supervised tracking model is able to deal with challenging scenarios, 
 such as large camera motion, occlusion and disocclusion, large deformation and scale variation.}
  \label{fig:qualitative}
\end{figure*}
% ===============
Extensive human annotations are required to achieve superior performance on dense tracking~(as shown in Figure~\ref{fig:teaser}),
for instance, an ImageNet~\cite{Deng09} pretrained ResNet is usually adopted as a feature encoder,
and further fintuned on a large number of images or frames with fine-grained, pixel-level segmentations, 
\eg COCO~\cite{Lin14}, Pascal~\cite{Everingham09a}, DAVIS~\cite{Pont-Tuset17} and YouTube-VOS~\cite{Xu18}.
Despite the rapid progress in dense tracking,
these supervised training seems very counter-intuitive when comparing with the development of human vision system.
It is known that human babies have already developed the ability for eye coordination and tracking by three months of age~\cite{Brazelton66, Kremenitzer79, Hofsten82}, 
in other words, 
the ability to track and follow slow-moving objects appears at a much earlier stage than being able to map objects to semantic meanings. 
With these evidences, it is unlikely the case that humans develop their tracking ability in a top-down manner, 
at least not at the early stage development of our vision systems.

In addition to the aforementioned approaches based on heavy supervision, 
several self-supervised methods~\cite{Vondrick18, Wang19, Lai19} have recently been proposed, 
leading more attractive directions for exploration since expensive semantic annotations are not required during training.
Unfortunately, none of the previous systems has demonstrated satisfactory results so far, 
they typically suffer from the problem from large deformation, fast motions, tracker drifting due to occlusions or disocclusions.
In this paper, we carefully examine the design choices in previous works~\cite{Vondrick18, Lai19}, 
pinpoint the potential flaws, and experimentally validate our conjectures to analyze the effects of core factors.

We make the following contributions:
First, 
we demontrate that channel dropout and jitterings are most effective
on $Lab$ color space, where the channels are decorrelated and reflect human perception. 
Second, to improve the training strategy, 
we spatially align the feature representation and downsampled image, 
train the models with photometric loss between the reconstructed and original frames,
naturally providing more discriminative training signals.
Third, we introduces a mechanism that allows hierarchical, dynamic memory mechanism.
To minimize the computational overhead and memory consumption,
we borrow the intuition from pre-attentive processing , 
\ie all available information in the previous video frames are coarsely processed, 
and information that has the highest salience or relevance is selected for further and more complete analysis by conscious (attentive) processing. 

We demonstrate that our method surpasses all existing self-supervised dense tracking methods by a significant margin on 
DAVIS-2017 and YouTube-VOS benchmarks~(Figure~\ref{fig:teaser}). 
Moreover, for the first time, 
we show that self-supervised learning on raw videos is able to produce competitive performance as those trained with heavy supervision.
While benchmarking on the unseen objects that not appearing in the training set, 
our model even outperform the heavily-engineered entries from the DAVIS competition winner,
demonstrating the usefulness and superior generalizability.
The goal of this paper is by no means to deny the necessity or the importance of supervised learning, 
instead, we try to demonstrate the potential of self-supervised dense tracking, 
and provide a strong baseline for future researches.

%On the other hand, state-of-the-art tracking by bounding box method typically adopt a siamese network based structure. 
%Such structure explores the translation-invariance property of CNNs and cast tracking into a similarity learning problem. 
%For example, [][] aims to compare an object template to sub-windows within the candidate image using shared-weight fully-convolutional conv-nets followed by a cross-correlation operation.

%In the same spirit of self-supervision, we propose a model that could be trained without any human supervision. 
%But we try to extend the previous methods by solving the aforementioned failure cases. Also, we propose a new memory mechanism to alliviate drifting and occlusion-related problems. As shown in Fig.~\ref{fig:teaser}, our model is able to achieve results comparable to many heavily supervised methods.



==> untitled folder/sec/intro_v2.tex <==
%!TEX root=../egpaper_for_review.tex

Although the working mechanisms of the human visual system remain somewhat obscure at the level of neurophysiology, 
it is a consensus that tracking objects is a fundamental ability that a baby starts developing at two to three months of age~\cite{Brazelton66, Kremenitzer79, Hofsten82}. 
Similarly, in computer vision systems, 
tracking plays key roles in a large number of applications ranging from autonomous driving to video surveillance. 

% =========================
\begin{figure}[t]
\includegraphics[width=0.5\textwidth]{figures/fig1.pdf}
\centering
\vspace{-0.5cm}
\caption{Comparison with other recent works on the DAVIS-2017 benchmark, 
\ie dense tracking or instance-wise video segmentation given the first frame annotation.
The proposed dense tracking system achieves state-of-the-art performance among all self-supervised approaches,
even comparable to some approaches trained with heavy supervision with ImageNet, COCO, Pascal, DAVIS, Youtube-VOS.\\
\textbf{Notation}:~CorrFlow~\cite{Lai19}, CycleTime~\cite{Wang19}, mgPFF~\cite{Song19}, Colorization~\cite{Vondrick18},
OSVOS~\cite{Caelles17}, VideoMatch~\cite{Hu18}, RGMP~\cite{Oh18}, OnAVOS~\cite{Voigtlaender17}, 
OSMN~\cite{Yang18}, FAVOS~\cite{Cheng18}, OSVOS-S~\cite{Maninis18}, FEELVOS~\cite{Voigtlaender19}, 
DyeNet~\cite{Li18ECCV}, PReMVOS~\cite{Luiten18}.}
\label{fig:teaser}
\vspace{-10pt}
\end{figure}
% =========================

Given arbitrary objects defined in the first frame, 
a tracking algorithm aims to relocate the same object throughout the entire video sequence. 
In the literature, 
tracking can be cast into two categories:
one is typically referred to as Visual Object Tracking (VOT)~\cite{VOT_TPAMI}, 
with the goal of relocalizing objects with bounding boxes throughout the video;
the other one aims for more fine-grained tracking, \ie relocalize the objects with pixel-level segmentation masks,
also known as Semi-supervised Video Object Segmentation (Semi-VOS)~\cite{Pont-Tuset17}.
In this paper, we focus on the latter case and refer to it as \emph{Dense Tracking} from here on. 

In order to achieve superior performance on such dense tracking task, 
recent methods usually require extensive manual annotations~(as shown in Figure~\ref{fig:teaser});
for instance, an ImageNet~\cite{Deng09} pre-trained ResNet is usually adopted as a feature encoder,
and further finetuned on a large number of images or frames with fine-grained, pixel-level semantic segmentation, 
\eg COCO~\cite{Lin14}, Pascal~\cite{Everingham09a}, DAVIS~\cite{Pont-Tuset17} and YouTube-VOS~\cite{Xu18}.
However, these supervised training schemes seem counter-intuitive when comparing to the development of the human vision system,
as human babies can track and follow slow-moving objects from two to three months of age, 
which is clearly a much earlier stage than being able to map objects to semantic meanings. 
With this evidence, 
it is unlikely the case that humans develop their tracking ability in a top-down manner~(supervised by semantics), 
at least not at the early stage development of the vision system.

% ===============
\begin{figure*}[!htb]
  \centering
%  % Requires \usepackage{graphicx}
  \includegraphics[width=.98\textwidth]{figures/qualitative_v3.pdf}
  \vspace{-3pt}
  \caption{\textbf{Train once, test on multiple datasets:}
Qualitative results from our \emph{self-supervised dense tracking model} on DAVIS-2017 and YouTube-VOS dataset. 
The number on the top left refers to the frame number in the video.
For all examples, the mask for $0th$ frame is given, and the task is to track the objects along with the video.
Our self-supervised tracking model is able to deal with challenging scenarios, 
such as large camera motion, occlusion and disocclusion, large deformation and scale variation.}
\label{fig:qualitative}
\end{figure*}
% ===============

In addition to the aforementioned approaches based on heavy supervision, 
several self-supervised methods~\cite{Vondrick18, Wang19, Lai19} have recently been proposed, 
leading to more attractive directions for exploration since expensive semantic annotations are not required during training.
Such self-supervised tracking algorithms have been proved possible without any finetuning.  
This differs from the self-supervised setting for other tasks, 
\eg~classification, which trains only the feature representation, 
and a final classification layer is still required to finetune on the full dataset with ground truth annotations. 
Self-supervised visual tracking algorithms\cite{Vondrick18,Wang19,Lai19,Wang19_Tracking}, 
on the other hand, are complete and do not require such a finetuning step.  

The most popular framework among these self-supervised tracking algorithms is based on feature similarity, 
\ie~label of the query pixel is assigned by the nearest reference pixels in the embedding space.
In this work, we argue in the same line and extend the idea of~\textit{correspondence flow} proposed by~\cite{Lai19}. 
Correspondence flow replaces traditional optical flow by relaxing the brightness constancy constraint and spatial smoothness,
allowing each query pixel to have correspondence with multiple reference pixels.
This representation turns out to be suitable for self-supervised dense tracking and has been shown to provide a huge performance gain over that based on optical flow. 

However, we identify a key issue of the method: 
the existing correspondence flow does not model large movement, 
since the query pixel can only look for similarities within a reference patch that is always placed around the query pixel. 
Motivated by this shortcoming, 
we add an offset to the representation and thus allow the patch to be non-locally placed, 
enabling the model to search for the reference patch dynamically.
We call this augmented representation, the \textit{non-local correspondence flow}. 

Building on our new non-local correspondence flow, 
we augment the tracking system proposed in \cite{Lai19} with a pre-attentive memory mechanism 
which allows to firstly make fixations to both long term and short term memories, 
and process the attended regions with a more complete analysis.
We show this is essential for dealing with the problems of large motion and occlusion in visual tracking, 
thus avoiding the complex training pipeline for handling tracker drift introduced in \cite{Lai19}. 
Our entire network, which we call \emph{Self-supervised Non-local Tracking Network (SNTNet)}, 
can be trained end-to-end on raw videos without any human annotation.

We evaluate SNTNet on multiple benchmarks for dense tracking with several compelling discoveries: 
First, our algorithm surpasses all existing self-supervised dense tracking methods by a significant margin on DAVIS-2017 ($13\%$) and YouTube-VOS ($20\%$) benchmarks, making SNTNet competitive with supervised methods. 
Second, we find that the model trained only on a small set of videos has already shown superior generalization capabilities on unseen objects and scenes. 
On the YouTube-VOS benchmark, we comfortably surpass PreMVOS~\cite{Luiten18}, 
the 2018 challenge winner algorithm trained with massive annotated datasets, on unseen object classes. 
Finally, we propose new training strategies with more effective losses and decorrelated color space,
which significantly improve the tracking performance, 
yielding state-of-the-art performance without using any human annotations.

==> untitled folder/sec/intro_v3.tex <==
%!TEX root=../egpaper_for_review.tex
% =========================
\begin{figure}[t]
\includegraphics[width=0.45\textwidth]{figures/fig1.pdf}
\centering
\vspace{-0.25cm}
\caption{Comparison with other recent works on the DAVIS-2017 benchmarks,
\ie dense tracking or semi-supervised video segmentation given the first frame annotation.
The proposed approach significantly outperforms the other self-supervised approaches, 
and even comparable to approaches trained with heavy supervision on ImageNet, COCO, Pascal, DAVIS, Youtube-VOS. 
In the x-axis, we only count pixel-wise segmentation.\\
\textbf{Notation}:
CINM~\cite{Bao18},
OSVOS~\cite{Caelles17}, 
AGAME~\cite{Johnander19},
VOSwL~\cite{Khoreva18},
FAVOS~\cite{Cheng18},
mgPFF~\cite{Song19}, 
CorrFlow~\cite{Lai19}, 
DyeNet~\cite{Li18ECCV}, 
PReMVOS~\cite{Luiten18}.
OSVOS-S~\cite{Maninis18}, 
RGMP~\cite{Oh18},
RVOS~\cite{Ventura19},
FEELVOS~\cite{Voigtlaender19}, 
OnAVOS~\cite{Voigtlaender17}, 
Video Colorization~\cite{Vondrick18},
SiamMask~\cite{Wang19a},
CycleTime~\cite{Wang19}, 
RANet~\cite{Wang19RA},
OSMN~\cite{Yang18}, 
}
\label{fig:teaser}
\vspace{-15pt}
\end{figure}
% =========================

% ===============
\begin{figure*}[!htb]
  \centering
%  % Requires \usepackage{graphicx}
  \includegraphics[width=.95\textwidth]{figures/qualitative_v5.pdf}
  \vspace{-3pt}
  \caption{\textbf{Train once, test on multiple datasets:}
Qualitative results from our \emph{self-supervised dense tracking model} on DAVIS-2017 and YouTube-VOS dataset. 
The number on the top left refers to the frame number in the video.
For all examples, the mask of the $0th$ frame is given, and the task is to track the objects along with the video.
Our self-supervised tracking model is able to deal with challenging scenarios, 
such as large camera motion, occlusion and disocclusion, large deformation and scale variation.}
\label{fig:qualitative}
\vspace{-15pt}
\end{figure*}
% ===============

%% Introduce importance of task
Although the working mechanisms of the human visual system remain somewhat obscure at the level of neurophysiology, 
it is a consensus that tracking objects 
is a fundamental ability that a baby starts developing at two to three months of age~\cite{Brazelton66, Kremenitzer79, Hofsten82}. 
Similarly, in computer vision systems, 
tracking plays key roles in many applications ranging from autonomous driving to video surveillance. 

%% Define task
Given arbitrary objects defined in the first frame, 
a tracking algorithm aims to relocate the same object throughout the entire video sequence. 
In the literature, 
tracking can be cast into two categories:
the first is Visual Object Tracking (VOT)~\cite{VOT_TPAMI}, 
where the goal is to relocalize objects with bounding boxes throughout the video;
the other aims for more fine-grained tracking, 
\ie~relocalize the objects with pixel-level segmentation masks,
also known as Semi-supervised Video Object Segmentation (Semi-VOS)~\cite{Pont-Tuset17}.
In this paper, 
we focus on the latter case, 
and will refer to it interchangeably with \emph{dense tracking} from here on. 

%% Explain existing supervised approaches
In order to train such dense tracking systems, 
most recent approaches rely on supervised training with extensive human annotations~(see Figure~\ref{fig:teaser}).
For instance, an ImageNet~\cite{Deng09} pre-trained ResNet~\cite{He16} is typically adopted as a feature encoder,
and further fine-tuned on images or video frames annotated with fine-grained, pixelwise segmentation masks, 
\eg COCO~\cite{Lin14}, Pascal~\cite{Everingham09a}, DAVIS~\cite{Pont-Tuset17} and YouTube-VOS~\cite{Xu18}.
Despite their success, 
this top-down training scheme seems counter-intuitive when considering the development of the human visual system,
as infants can track and follow slow-moving objects before they are able to map objects to semantic meanings. 
With this evidence, 
it is unlikely the case that humans develop their tracking ability in a top-down manner~(supervised by semantics), 
at least not at the early-stage development of the visual system.

%% Introduce self-supervised methods
In contrast to the aforementioned approaches based on heavy supervision, 
self-supervised methods~\cite{Vondrick18, Wang19, Lai19, Wang19_Tracking} have recently been introduced, 
leading to more neurophysiologically intuitive directions.
While not requiring any labeled data, the performance of these methods is still far from that of supervised methods (Figure~\ref{fig:teaser}).
%These approaches stand in contrast to the classical self-supervised setting on other vision tasks.
%For example, self-supervised classification algorithms can only provide a feature representation and
%a final classification layer still requires extensive finetuning on the full dataset with ground truth annotations. 
%The aforementioned self-supervised visual tracking algorithms,
%on the other hand, are complete and can be deployed on downstream tracking tasks \textbf{with no finetuning}.  

%The most popular framework among these self-supervised tracking algorithms relies on feature similarity, 
%\ie~label of the query pixel is assigned by the `nearest' reference pixels in the embedding space.
%However, the computational complexity of this pixel comparison procedure typically scales in degree 4
%with the image resolution in space and degree 5 in spacetime\cite{Wang2018}. 
%In order to retrieve high-resolution information from a memory bank without hitting a computational bottleneck,
%we propose a novel attention mechanism in this work, which scales only in degree 2 (space) or degree 3 (spacetime).

%% Introduce our improved method
We continue in the vein of self-supervised methods and propose an improved tracker,
which we call \emph{Memory-Augmented Self-Supervised Tracker} (MAST).
Similar to previous self-supervised methods, 
our model performs tracking by learning a feature representation that enables robust pixel-wise correspondences between frames; 
it then propagates a given segmentation mask to subsequent frames based on the correspondences. 
We make three main contributions:
\emph{first},
we reassess the traditional choices used for self-supervised training and reconstruction loss 
by conducting thorough experiments to finally determine the optimal choices. 
\emph{Second}, to resolve the challenge of tracker drift (\ie~as the object changes appearance or becomes occluded,
each subsequent prediction becomes less accurate if propagated only from recent frames),
we further improve on existing methods by augmenting our architecture with a crucial memory component. 
We design a coarse-to-fine approach that is necessary to efficiently access the memory bank:
%To avoid increasing computation from calculating correspondences with many frames,
a two-step attention mechanism first coarsely searches for candidate windows,
and then computes fine-grained matching.
We conduct experiments to analyze our choice of memory frames,
showing that both short- \emph{and} long-term memory
are crucial for good performance.
\emph{Third}, 
we benchmark on large-scale video segmentation datasets and propose a new metric, \emph{i.e.}~generalizability,
with the goal of measuring the performance gap between tracking seen and unseen categories, 
which we believe better captures the real-world use-cases for category-agnostic tracking.

The result of the first two contributions 
is a self-supervised network that surpasses 
all existing approaches by a significant margin on DAVIS-2017 ($15\%$) and YouTube-VOS ($17\%$) benchmarks,
making it competitive with supervised methods \emph{for the first time}.
Our results show that a strong representation for tracking can be learned without using any semantic annotations,  
echoing the early-stage development of the human visual system.
Beyond significantly narrowing the gap with supervised methods on the existing metrics,
we also demonstrate the \emph{superiority} of self-supervised approaches over supervised methods on generalizability.
On the unseen categories of YouTube-VOS benchmark, 
we surpass PreMVOS~\cite{Luiten18}, 
the 2018 challenge winner algorithm trained on massive segmentation datasets.
Furthermore, when we analyze the drop in performance between seen and unseen categories,
we show that our method (along with other self-supervised methods) has a significantly smaller
\emph{generalization gap} than supervised methods.
These results show that contrary to the popular belief that self-supervised methods are not yet useful
due to their weaker performance, 
their greater generalization capability (due to not being at risk of overfitting to labels)
is actually a more desirable quality when being deployed in real-world settings,
where the domain gap can be significant.


%We first revisit the various choices made in previous works and conduct thorough ablation studies
%to clarify the design choices that yield the richest self-supervision signals.
%Second, we introduce a novel memory module to counter the infamous tracker drift problem.


%Specifically, we propose a \emph{deformable attention},
%in which a memorized frame is only coarsely processed at the initial stage,
%regions with the highest salience or relevance~(a stimulus that stands out the most) to a query are further selected 
%for more complete analysis by conscious~(attentive) processing. 
%
%Memory and attention are two closely related key features that enable many of our fundamental cognitive abilities. 
%For example, we use attention to prioritize important part of the memory to better achieve certain ends and address bottlenecks in information processing capacity.
%Recently, communities such as vision and language have taken this observation and adopted attention-based networks for modeling long-range dependencies (\eg~\cite{Bahdanau2015,Wang2018,Vaswani17,Seoung19,Devlin18}). These algorithms have the ability to attend to different positions in time, and have been shown to  yield to state-of-the-art performance in many applications. 


%Building on this attention mechanism, our entire ne% However, this doesn't tell the rk, which we call \emph{Self-supervised Memory Augmented Tracker (SMAT)}, 
%is trained end-to-end on raw videos and evaluated on multiple benchmarks for dense tracking with several compelling discoveries: 
%first, the representation for tracking can indeed be learnt without using any semantic annotations,  
%echoing the early-stage development of the human vision system.
%SMAT surpasses all existing self-supervised dense tracking methods by a significant margin on DAVIS-2017 ($15\%$) and YouTube-VOS ($20\%$) benchmarks, making it competitive with supervised methods. 
%Second, the model trained only on a small set of videos has already shown superior generalizability on unseen objects and scenes. 
%On the YouTube-VOS benchmark, we comfortably surpass PreMVOS~\cite{Luiten18}, 
%he 2018 challenge winner algorithm trained with massive segmentation datasets, on unseen object classes. 
%Finally, we describe new training strategies with more effective losses and decorrelated color space,
%which significantly improve the tracking performance, 
%yielding state-of-the-art performance without using any human annotations.


% Specifically, we propose a attention mechanism based on the idea of~\textit{correspondence flow} proposed by~\cite{Lai19}. 
% Correspondence flow replaces traditional optical flow by relaxing the brightness constancy constraint and spatial smoothness,
% allowing each query pixel to have correspondence with multiple reference pixels.
% This representation turns out to be suitable for self-supervised dense tracking and has been shown to provide a huge performance gain over that based on optical flow. 

% However, we identify a key issue of the method: 
% the existing correspondence flow does not model large movement, 
% since the query pixel can only look for similarities within a reference patch that is always placed around the query pixel. 
% Motivated by this shortcoming, 
% we add an offset to the representation and thus allow the patch to be non-locally placed, 
% enabling the model to search for the reference patch dynamically.
% We call this augmented representation, the \textit{non-local correspondence flow}. 

% Building on our new non-local correspondence flow, 
% we augment the tracking system proposed in \cite{Lai19} with a pre-attentive memory mechanism 
% which allows to firstly make fixations to both long term and short term memories, 
% and process the attended regions with a more complete analysis.
% We show this is essential for dealing with the problems of large motion and occlusion in visual tracking, 
% thus avoiding the complex training pipeline for handling tracker drift introduced in \cite{Lai19}. 


==> untitled folder/sec/method.tex <==
%!TEX root=../egpaper_for_review.tex
\section{Method}
% {\color{red} TODO: add overview: 1) background, 2) improvements, 3) tracker}
The proposed dense tracking system, 
MAST (Memory-Augmented Self-Supervised Tracker), 
is a conceptually simple model for dense tracking that can be trained with self-supervised learning,
\ie \textbf{zero manual annotation} is required during training,
and an object mask is only required for the first frame during inference.
In Section~\ref{sec:background},
we provide relevant background of previous self-supervised dense tracking algorithms,
and terminologies that will be used  in later sections.
Next, in Section~\ref{sec:training_signal}, 
we pinpoint weaknesses in these works and propose improvements to the training signals.
Finally, in Section~\ref{sec:memory}, we propose memory augmentation as an extension to existing self-supervised trackers.

%
\subsection{Background}
\label{sec:background}
In this section,
we review previous papers that are closely related to this work~\cite{Vondrick18, Lai19}.
In general, 
the goal of self-supervised tracking is to learn feature representations that enable robust correspondence matching.
During training, 
a proxy task is posed as reconstructing a target frame~($I_t$) by linearly combining pixels from a reference frame~($I_{t-1}$),
with the weights measuring the strength of correspondence between pixels.

Specifically, 
a triplet~($\{Q_t, K_t, V_t\}$) exists for each input frame $I_t$, 
referring to \emph{Query}, \emph{Key}, and \emph{Value}.
In order to reconstruct a pixel $i$ in the $t$-th frame~($\hat{I^i_t}$),
an \textit{Attention} mechanism is used for \emph{copying} pixels from a subset of previous frames in the original sequence.
This procedure is formalized as:
\begin{align} 
\label{eq:attention}
  \hat{I^i_t} = \sum _{j} A^{ij}_{t} V^j_{t-1} \\
\label{eq:affinity}
  A^{ij}_t =  \frac{exp\langle\ Q_t^i,K_{t-1}^j\rangle}{\sum_p exp\langle\ Q_t^i,K_{t-1}^p\rangle}
\end{align}

\noindent where $\langle\cdot,\cdot\rangle$ refers to the dot product between two vectors, 
query~(Q) and key~(K) are feature representations computed by 
passing the target frame $I_t$ to a Siamese ConvNet $\Phi(\cdot; \theta)$, 
\ie $Q_t = K_t = \Phi(I_t; \theta)$,
$A_t$ is the affinity matrix representing the feature similarity between pixel $I^i_t$ and $I^j_{t-1}$,
value~(V) is the raw reference frame~($I_{t-1}$) during the training stage, 
and instance segmentation mask during inference,
achieving reconstruction or dense tracking respectively.

A key element in self-supervised learning is to set the proper \emph{information bottleneck},
or the choice of what input information to withhold for learning the desired feature representation 
and avoiding trivial solutions.
For example, in the reconstruction-by-copying task,
an obvious shortcut is that the pixel in $I_t$ can learn to match any pixel in $I_{t-1}$ with the \emph{exact same color}, 
yet not necessarily correspond to the same object.
To circumvent such learning shortcuts,
Vondrick \etal~\cite{Vondrick18} intentionally drop the color information from the input frames.
Lai and Xie~\cite{Lai19} further show that a simple channel dropout can be more effective.

% ------------------
\subsection{Improved Reconstruction Objective} 
\label{sec:training_signal}
% ------------------
In this section,
we reassess the choices made in previous self-supervised dense tracking works and provide intuition for our optimal choices,
which we empirically support in Section \ref{sec:experiments}.
% ===============
\vspace{-5pt}
\subsubsection{Decorrelated Color Space}
\label{sec:color}
% ------------------
Extensive experiments in the human visual system have shown that colors can be seen as combinations of the primary colors,
namely red (R), green (G) and blue (B).
For this reason, 
most of the cameras and emissive color displays represent pixels as a triplet of intensities:~$(R,G,B) \in \mathcal{R}^3$.
However,
a disadvantage of the RGB representation is that the channels tend to be extremely correlated~\cite{Reinhard01},
as shown in Figure~\ref{fig:color}.
In this case, 
the channel dropout proposed in~\cite{Lai19} is unlikely to behave as an effective information bottleneck,
since the dropped channel can almost always be determined by one of the remaining channels.

% ===============
\begin{figure}[!h]
  \centering
  \includegraphics[width=.45\textwidth]{figures/colorspace_v7.pdf}
  \vspace{-2pt}
  \caption{Correlation between channels of RGB and $Lab$ colorspace. 
We randomly take $100,000$ pixels from 65 frames in a sequence~(snowboard) in the DAVIS dataset and plot the relative relationships between RGB channels. This phenomena generally holds for all natural images~\cite{Reinhard01}, 
due to the fact that all of the channels include a representation of brightness.
Values are normalized for visualization purposes.}
  \label{fig:color}
\end{figure}
% ===============

To remedy this limitation,
we hypothesize that dropout in the decorrelated representations~(\eg~$Lab$) 
would force the model to learn invariances suitable for self-supervised dense tracking;
\ie if the model cannot predict the missing channel from the observed channels,
it is forced to learn a more robust representation rather than relying on local color information.
%for instance, if the color of one input channel is unpredictable from the others, 
%yet the model is still capable to matching the correspondence and copying colors from a reference frame, 
%it must have learnt more robust representations that are invariant to the low-level colors.
%In Section~\ref{exp:ablation}, 
%we validate our conjecture that channel-wise dropout
%are indeed more effective on input frames represented in the $Lab$ color space,
%which separates luminance and chrominance, resulting in low mutual information.

% ------------------
\vspace{-5pt}
\subsubsection{Classification vs. Regression}
\label{sec:loss}
% ------------------
In the recent literature on colorization and generative models~\cite{Zhang16_Color,Oord16},
colors were quantized into discrete classes and treated as a multinomial distribution,
since generating images or predicting colors from grayscale images is usually a non-deterministic problem; 
\eg the color of a car can reasonably be red or white.
However, this convention is suboptimal for self-supervised learning of correspondences,
as we are not trying to generate colors for each pixel,
but rather, estimate a precise relocation of pixels in the reference frames.
More importantly,
quantizing the colors leads to an information loss that can be crucial for learning high-quality correspondences.

We conjecture that directly optimizing a regression loss between the reconstructed frame~($\hat{I_{t}}$) and real frame~($I_t$) will provide more discriminative training signals.
In this work, the objective $\mathcal{L}$ is defined as the Huber Loss:
\begin{align}
\mathcal{L} = \frac{1}{n} \sum_{i} z_{i}
\end{align}
\vspace{-.3cm}
\noindent where
\begin{align}
 z_{i} =
        \begin{cases}
        0.5 (\hat{\textbf{I}}^i_t - \textbf{I}^i_t)^2, & \text{if } |\hat{\textbf{I}}^i_t - \textbf{I}^i_t| < 1 \\
        |\hat{\textbf{I}}^i_t - \textbf{I}^i_t| - 0.5, & \text{otherwise }
        \end{cases}
\end{align}
where $\hat{\textbf{I}}^i_t \in \mathcal{R}^3$ refers to RGB or \emph{Lab}, 
normalized to the range [-1,1] in the reconstructed frame that is copied from pixels in the reference frame~$I_{t-1}$,
and $I_t$ is the real frame at time point $t$.

% ------------------

\begin{figure*}[!htb]
  \centering
  \includegraphics[width=.98\textwidth]{figures/scheme_v10.pdf}
  \vspace{-3pt}
  \caption{Structure of MAST. 
  The current frame is used to compute \textbf{query} to attend and retrieve from memory (\textbf{key} \& \textbf{value}). 
  During training, we use raw video frame as \textbf{value} for self-supervision. 
  Once the encoder is trained, we use instance mask as \textbf{value}. See Section~\ref{sec:memory} for details.}
  \vspace{-5pt}
  \label{fig:scheme}
\end{figure*}
% ------------------

\vspace{5pt}
\subsection{Memory-Augmented Tracking}
\label{sec:memory}
% {\color{red} Todo: transition}
So far we have discussed the straightforward attention-based mechanism for propagating
a mask from a single previous frame.
However, as predictions are made recursively,
errors caused by object occlusion and disocclusion tend to accumulate 
and eventually degrade the subsequent predictions.
To resolve this issue, we propose an attention-based tracker that efficiently makes use of \emph{multiple} reference frames. 

\subsubsection{Multi-frame tracker}
An overview of our tracking model is shown in Figure~\ref{fig:scheme}.
To summarize the tracking process: 
given the present frame and multiple past frames (memory bank) as input,
we first compute the query~(Q) for the present frame and keys~(K) for all frames in memory.
Here, we follow the general procedure in previous works as described in Section~\ref{sec:background},
where K and Q are computed from a shared-weight feature extractor and
V is equal to the input frame (during training) or object mask (during testing).
The computed affinity between Q and all the keys~(K) in memory is 
then used to make a prediction for each query pixel depending on V.
Note we don't put any weights on the reference frames,
as this should be encoded in the affinity matrix 
(\emph{e.g.}~when a target and reference frame are dis-similar,
the corresponding similarity value will be naturally low;
thus the reference label will have less contribution to the labeling of a target pixel).

The decision of which pixels to include in K is crucial for good performance.
Including all pixels previously seen is far too computationally expensive due to the quadratic explosion of the affinity matrix (\eg
the network of~\cite{Lai19} produces affinity matrices with more than 1 billion elements for 480p videos).
To reduce computation, 
\cite{Lai19} exploit temporal smoothness in videos and apply restricted attention, 
only computing the affinity with pixels in a ROI around the query pixel location.
However, the temporal smoothness assumption holds only for temporally close frames.

To efficiently process temporally distant frames, we propose a two-step attention mechanism.
The first stage involves coarse pixel-matching with the frames in the memory bank to
determine which ROIs are likely to contain good matches with the query pixel.
In the second stage, we extract the ROIs and compute fine-grained pixel matching,
as described in Section~\ref{sec:background}.
Overall, the process can be summarized in Algorithm~\ref{algorithm}.
\setlength{\textfloatsep}{2pt}% Remove \textfloatsep
\begin{algorithm}[!htb]
\small
  \caption{MAST} 
  \begin{algorithmic}[1]
    \State Choose $m$ reference frames $Q_1, Q_2, ... Q_m$
    \State Localize ROI $R_1, R_2, ... R_m$ according to 3.3.2 (Eq. 5 and 6) for each of the reference frames 
    \State Compute similarity matrix $A^{ij}_t = \langle Q^j,R_t^i\rangle $  between target frame $Q$ and each ROI.
%    \State Normalize $A_{1..m}$ so that they altogether sum up to 1. 
    \State Output: pixel's label is determined by aggregating the labels of the ROI pixels (weighted by its affinity score).
  \end{algorithmic} 
\label{algorithm}
\end{algorithm}

\vspace{-15pt}
\subsubsection{ROI Localization}
\label{sec:localization}
The goal of ROI localization is to estimate the candidate windows non-locally from memory banks. As shown in Figure~\ref{fig:ROI}, this can be achieved through restricted attention with varying dilation rate.

Intuitively, for short-term memory (temporally close frames),
dilation is not required since spatial-temporal coherence naturally exists in videos;
thus ROI localization becomes restricted attention~(similar to \cite{Lai19}).
However, for long-term memory,
we aim to account for the fact that objects can potentially appear anywhere in the reference frames.
We unify both scenarios into a single framework for learning ROI localization.
% ===============
\begin{figure}[H]
  \centering
%  % Requires \usepackage{graphicx}
  \includegraphics[width=.42\textwidth]{figures/NCF_v1.pdf}
  \vspace{-3pt}
  \caption{ROI Localization.}
  \label{fig:ROI}
\end{figure}
% ===============

Formally, for the query pixel $i$ in $I_t$, to localize the ROI from frame~($I_{t-N}$),
%the initial process can be described as:
we first compute in parallel $H^i_{t-N, x,y}$, the similarity heatmap between $i$ and all candidate pixels in the dilated window:
\begin{align}
H^i_{t-N, x,y} = softmax(Q^i_t \cdot im2col(K^i_{t-N}, \gamma_{t-N}))
\end{align}
where $\gamma_{t-N}$ refers to the dilation rate for window sampling in frame $I_{t-N}$,
and $im2col$ refers to an operation that transforms the input feature map into a matrix based on dilation rate. 
Specifically, in our experiments, the dilation rate is proportional to the temporal distance between the present frame and the past frames in the memory bank, \ie~$\gamma_{t-N} \propto N$. 
We use $\gamma_{t-N} = \left \lceil (t-N)  / 15 \right \rceil$.

The center coordinates for ROIs can be then computed via a \textit{soft-argmax} operation:
\begin{align}
P^i_{x,y} = \sum_{x,y} H^i_{x,y} * C 
\end{align}
where $P^i_{x,y}$ is the estimated center location of the candidate window in frame $I_{t-N}$ for query pixel $I^i_t$,
and $C$ refers to the grid coordinates~($x,y$) corresponding to the pixels in the window from $im2col$.
The resampled Key~($\hat{K}^i_{t-N}$) for pixel $I^i_t$ can be extracted with a bilinear sampler~\cite{Jaderberg2015}.
With all the candidate Keys dynamically sampled from different reference frames of the memory bank, 
we compute fine-grained matching scores only with these localized Keys,
resembling a restricted attention in a non-local manner.
Therefore, with the proposed design, 
the memory-augmented model can efficiently access high-resolution information for correspondence matching, 
without incurring large physical memory costs.  

%\subsubsection{Why two-stage process}
%A basic solution for memory retrival is dot-product attention across all reference frames (Eq.~\ref{eq:attention} and \ref{eq:affinity}).
%However, this simple mechanism struggles for high-resolution tracking because of the quadratic explosion of the affinity matrix (\eg
%the network of~\cite{Lai19} produce affinity matrices with more than 1 billion elements on 480p videos).
%Although it allows memory retrival in theory, processing multiple such affinity matrices is simply computationally unrealistic.
%
%To exploit temporal smoothness in videos,
%\cite{Lai19} applies restricted attention,
%effectively placing the ROI around the query pixel.
%The authors show that the method yields better performances and is computationally-efficient - \eg
%reducing size of similarity matrices by two orders of magnitude.
%However,
%such restricted attention only works for close-by frames since large movement cannot be modelled.
%
%To get the best of both worlds, we borrow intuition from the classical coarse-to-fine process.
%The addition of ROI Localization module first coarsely filter frames in the memory bank, which is then processed for  fine-grained matching. By using the same window size, it models large movement without using any extra memory size compared to restricted attention.

% \subsubsection{Tracking from Multi-frames}
% {\color{red} Todo: add this section. explain technical details of making current prediction (\eg how to compute memory, multiple affinity matrix; how to warp multiple frames etc.). }


% \subsubsection{Matching \& Resampling}
% Once the ROIs are selected from multiple reference frames in the memory banks,
% the affinity matrix $A$ can be computed in a similar way to Eq.~\ref{eq:affinity},
% and the query pixel is reconstructed by a linear combination of all the pixels in the ROIs.
% Ideally, as objects can be occluded or disoccluded throughout the video,
% the query pixel will have a better chance of finding correspondences from the reference frames in the memory bank.


%we can use the pixel similarities to determine if the query pixel appears in the frame. 
%If a query pixel does not show up in a frame, the response in the ROI is all low. 
%In contrast, if a query pixel appear in a frame, 
%the response is high. 
%Since we aim to resample the query pixel from all memorized frames, 
%a simple solution is to find the weights to linearly combine the retrieved pixels and reconstruct the query pixel. 
%A natural solution is to find the weight is by applying a softmax acrossing both spatial and temporal dimension.

%\begin{align}
%A_{ijk} =  \frac{exp\langle\ f^i_t,f^j_k\rangle}{\sum_{jk} exp\langle\ f^i_t,f^j_{k}\rangle}
%\end{align}
%where $A$ stands for a similarity volume now.
%If the query pixel does not show up in some frames,
%the similarity of the entire frame is lower and the frame will be automatically ignored by the \textit{softmax} operation.

% \subsubsection{Bidirectional correspondence searching}
% When computing the reconstruction error, 
% the current methods only copy pixels from the previous frames.
% This can cause issues on pixels that are only visible in the curret frame, 
% but \emph{not visible} in any of the previous frames,
% Therefore, it violates the fundamental assumption that each pixel can be matched with pixels in previous frames,
% either introducing a high photometric loss or leading the model to compromise the matching performance, 
% and drift to other pixels in the neighborhood.
% These errors mainly come from two sources: pixels that are occluded or disoccluded, 
% and pixels at the boundary coming into the field of view.

% In fact, despite the time flows uni-directionally in the physical world, 
% there is no reason preventing us from exploring bidirectional correspondences in the videos.
% We can actually solve the aforementioned challenge by defining the loss as the minimum of bidrectional matching:
% \begin{align}
% L_p = min\{ L_{I_{t-1 \rightarrow t}},  L_{I_{t+1 \rightarrow t}} \}
% \end{align} 

%\subsection{Upperbound of Self-supervised Learning.}
%In order to demonstrate the power of self-supervised learning, 
%it is essential to train more powerful models.
%The model should at least be able to overfit the training set, 
%otherwise, we are not taking the core benefit of unsupervised learning.\\

%While checking the Table~3 in the BMVC paper,
%it is possible to outperform the supervised learning model with more diverse videos and models with higher capacity, \eg~ResNet-50, typical examples are.

%\subsection{Effectiveness of Finetuning on Dense Tracking.}
%\hl{Finetune the model with video segmentation masks, plot the relationships between the data for supervision and performance. }
%\vspace{0.5cm}

%\subsection{Instance Segmentation with the Self-supervised Representation}
%\hl{Take the learnt re. }
%\vspace{0.5cm}



% We propose a new attention function based on the restricted attention proposed , called \textit{deformable attention}. As shown in fig~\ref{fig:self_attention}, the new attention adds a component called \textit{ROI selection}, which estimate an offset from the given input. 


% Tracker drift remains a fundamental challenge for self-supervised dense tracking.
% As predictions are made recursively,
% errors caused by object occlusion and disocclusion tend to accumulate, 
% and eventually contaminate the subsequent predictions.
% In~\cite{Lai19},
% the authors proposed to alleviate the problem using scheduled sampling and forward-backward cycle consistency.

% In this section,
% we explore other possible solutions, \ie~augmenting the architecture with external memory modules.
% Specifically, we form a space-time non-local correspondence flow between the memory bank and the query image~(as shown in Figure~\ref{fig:scheme}). 
% Ideally, we want to enable each query pixel in the target frame to search all previous frames to find the optimal correspondence,
% however,
% this process is usually intractable as the memory required for computing the affinity matrix will grow quadratically.
% To strike a balance between computational cost and accuracy,
% %To obtain the offset value for each frame, 
% we take inspiration from pre-attentive processing,
% \ie information in previous video frames are coarsely processed to infer an offset for each query pixel, 
% and extract the regions with candidate reference pixels.
% These \emph{small regions} will therefore have the highest salience (a stimulus that stands out the most) or
% relevance to a query pixel, 
% and be bilinearly resampled from reference frames for attentive processing~(fine-grained correspondence matching).

% As an extension to the process described earlier~(Section~\ref{sec:background}),
% multiple reference frames from both long term~($I_{t-N}$, $N$ refers to the temporal gap)
% and short term memory~($I_{t-1}$) are fed as inputs to reconstruct the target frame~($I_t$).
% In the following sections,
% we describe the two core components that form the non-local correspondence flow:
% \textbf{ROI Localization} and \textbf{Matching \& Resampling}.

% %We then obtain all pixels in the query image by resampling from frames in the memory bank based on feature similarity. 
% %First, we estimate a rough region of interest (ROI), 
% %which is the most possible region that the query pixel resides in the corresponding frames. 
% %Next, instead of generating independent current frame prediction, 
% %we compute a single dot-product similarity volume between all ROIs and the query pixel. 
% %Finally, this volume is softmaxed and the query pixel is resampled as a linear combination
% %(weighted by aforementioned similarities) of pixels in all RoIs.  

% %\subsubsection{Non-local Correspondence Flow}
% %Figure~\ref{fig:Flow} illustrates the augmented correspondence flow, 
% %which is used to reconstruct the current frame with earlier frames. 
% %The non-local correspondence flow extends the correspondence flow with an offset, 
% %so that the representation could be used to model large movements. 
% %Taking two frames as input, ROI Localization first estimate the offset. 
% %A region of interest(ROI) is then extracted with a bilinear sampler at the offset location. 
% %Multiple such ROIs are extracted from several frames in the memory bank and used to match and resample the current pixel. 

% %
% % ===============
% %\begin{figure}[H]
% %  \centering
% %  % Requires \usepackage{graphicx}
% %  \includegraphics[width=.45\textwidth]{figures/flow_v1.pdf}
% %  \vspace{-3pt}
% %  \caption{Non-local Correspondence Flow. See text for details. }
% %  \label{fig:Flow}
% %\end{figure}
% % ===============



==> untitled folder/sec/method_v0.tex <==
%!TEX root=../egpaper_for_review.tex
\section{Method}
% {\color{red} TODO: add overview: 1) background, 2) improvements, 3) tracker}
The proposed dense tracking system, 
MAST (Memory-Augmented Self-supervised Tracker), 
is a conceptually simple model for dense tracking that can be trained with self-supervised learning,
\ie \textbf{zero manual annotation} is required during training,
and an object mask is only required for the first frame during inference.
In Section~\ref{sec:background},
we provide relevant background of previous self-supervised dense tracking algorithms,
and termonologies that will be used  in later sections.

Next, in Section~\ref{sec:training_signal}, 
we pinpoint weaknesses in these works and propose improvements to the training signals.
Finally, in Section~\ref{sec:memory}, we propose memory augmentation as an extension to existing self-supervised trackers.

%
\subsection{Background}
\label{sec:background}
% {\color{red} Todo: make background section more concise, especially last paragraph.}
%\begin{figure}[!h]
%  \centering
%  \includegraphics[width=.45\textwidth]{figures/background.pdf}
%  \vspace{-2pt}
%  \caption{\textbf{Correspondence from frame reconstruction}: The correspondence can be learned from reconstructing target from the reference frame. After the correspondence is learned, it can be used to track arbitrary objects.}
%  \label{fig:background}
%\end{figure}

In this section,
we review previous works that are closely related~\cite{Vondrick18, Lai19}.
The goal of self-supervised tracking is to learn robust feature representations that enables robust correspondence matching.
During training, 
the proxy task is posed as reconstructing a target frame~($I_t$) by ``copying''~(linearly combining) pixels from $I_{t-1}$,
where the correspondence between pixels in target frame and reference frame is computed with \emph{Attention} mechanism. 
%a learned feature extractor (Fig.~3 encoder) produces representations suitable for correspondence matching are learned as a byproduct from \textit{frame reconstruction}. 

%This process can be understood in the general framework of (self-)attention~\cite{Vaswani17},
%that is designed for Seq2Seq problems:
%an input sequence (original video sequence), \eg~$S_{input}=\{I_t\}_{t=1}^n$
%is used to predict an output sequence (reconstructed video sequence), \eg~$S_{output}=\{\hat{I}_t\}_{t=1}^n$.

Specifically, a triplet~($\{Q_t, K_t, V_t\}$) exists for each input frame $I_t$, 
referring to \emph{Key}, \emph{Query}, and \emph{Value}.
In order to reconstruct a pixel $i$ in the $t$-th frame~($\hat{I^i_t}$),
an \textit{Attention} mechanism is used for  \emph{soft-copying} pixels from a subset of previous frames in the original sequence,
this procedure is formalized as
\begin{align} 
\label{eq:attention}
  \hat{I^i_t} = \sum _{j} A^{ij}_{t} V^j_{t-1} \\
\label{eq:affinity}
  A^{ij}_t =  \frac{exp\langle\ Q_t^i,K_{t-1}^j\rangle}{\sum_p exp\langle\ Q_t^i,K_{t-1}^p\rangle}
\end{align}

\noindent where $\langle\cdot,\cdot\rangle$ refers to the dot product between two vectors,
and $A_t$ is the affinity matrix representing the feature similarity between pixel $I^i_t$ and $I^j_{t-1}$.
In these works, query~(Q) and key~(K) are feature representations computed by 
passing the target frame $I_t$ to the same deep ConvNet $\Phi(\cdot; \theta)$, 
\ie $Q_t = K_t = \Phi(I_t; \theta)$. 
Value~(V) is the raw reference frame~($I_{t-1}$) during the training stage, 
and instance segmentation mask during inference.


% Here, the underlying assumption is that the pixel in the current frame can be reconstructed by a linear combination of all pixels in the previous frame. 
% As an improvement, \cite{Lai19} argues that this assumption is unnecessary because objects always move locally between frames. 
% Therefore, they propose to use \textit{correspondence flow} to 
% reconstruct each query pixel by linear combinations of the reference pixels in a window with restricted size.
% This representation has been shown to achieve state-of-the-art performance in self-supervised dense tracking.

A key element in self-supervised learning is the \emph{information bottleneck},
or the decision of what input information to withhold to learn a good feature representation
and to avoid learning trivial solutions.
For example, in the frame reconstruction task,
an obvious shortcut is that the pixel in $I_t$ can learn to match any pixel in $I_{t-1}$ with the \emph{exact same color}, 
yet not necessarily share any semantic similarity.
%Another concern is to avoid trivial solutions during training; in other words, if training is done na\"ively,
%it is not guaranteed to obtain feature representations for high-quality correspondence matching.
%An obvious shortcut is that the pixel in $I_t$ can learn to match any pixel in $I_{t-1}$ with the \emph{exact same color}, yet not necessarily share any semantic similarity.
To circumvent such learning shortcuts,
Vondrick \etal~\cite{Vondrick18} intentionally drop the color information from the input frames.
Lai and Xie~\cite{Lai19} further show that a simple channel dropout can be effective.

% With the learnt affinity matrix,
% the downstream dense tracking is therefore posed as mask propagation from $M_{t-1}$~(instance mask of $I_{t-1}$):
% \begin{align}
% M^{i}_t = \sum_{j} A_{ij} M^j_{t-1}
% \label{eq:prop}
% \end{align}

% $\Phi(\cdot; \theta)$ is a deep ConvNet.

% the query~(Q) refers to the pixelwise feature representation computed from the current frame, \ie $f_t$;
% the key~(K) refers to the feature representation of the reference frame, \ie $f_{t-1}$,
% while value~(V) denotes the raw reference frame~($I_{t-1}$) during the training stage, 
% and instance segmentation mask~($M_{t-1}$) during inference.
% For simplicity, we will stick on this set of notations in the following sections.

% % Formally,
% % assume we are given two frames from a video~$I_{t-1}$ and $I_t$~($t-1$ and $t$ refer to the time point).
% % ,
% % then a feature encoder $f$ is parametrized by a ConvNet, denoted as $\Phi(\cdot; \theta)$:
% % \begin{align}
% % f_{t-1}, f_t = \Phi(I_{t-1}; \theta), \Phi(I_t; \theta)
% % \end{align}
% % The goal is to enable every pixel in $I_t$ to find its counterpart in frame $I_{t-1}$,
% % which share the same semantics.
% % Notice objects generally move smoothly and appearance will not change abruptly, so we assume frame $I_t$ can be reconstructed purely by ``copying'' pixels from $I_{t-1}$,
% % correspondence matching has been learnt.
% % In \cite{Vondrick18}, this intuition is formalized as :
% \begin{align}
% \hat{I^i_t} = \sum _{j} A_{ij} I^j_{t-1} \text{\hspace{.25cm}
% where\hspace{.1cm}} A_{ij} =  \frac{exp\langle\ f^i_t,f^j_{t-1}\rangle}{\sum_k exp\langle\ f^i_t,f^k_{t-1}\rangle}
% \label{eq:affinity}
% \end{align}
% %
% where $\hat{I^i_t}$ refers to the reconstructed frame for $I_t$,
% $\langle\cdot,\cdot\rangle$ refers to the dot product between two vectors,
% and $A$ is the affinity matrix with each element representing the pairwise pixel similarity,
% \eg\ $A_{ij}$ denotes the correspondence between pixel $I^i_t$ and $I^j_{t-1}$. 
% The underlying assumption is that the pixel in the current frame can be reconstructed by a linear combination of all pixels in the previous frame. 
% As an improvement, \cite{Lai19} argues that this assumption is unnecessary because objects always move locally between frames, 
% \ie the natural spatial-temporal consistency in videos. 
% Therefore, they propose to use \textit{correspondence flow} that 
% reconstructs each query pixel by linear combinations of the reference pixels in a window with restricted size.
% This representation has been shown to yield state-of-the-art performance in self-supervised dense tracking.

% Another concern is to avoid trivial solutions during training, in other words, if training is done na\"ively,
% it is not guaranteed to obtain feature representations for high-quality correspondence matching.
% An obvious shortcut is that the pixel in $I_t$ can learn to match any pixel in $I_{t-1}$ with the \emph{exact same color}, yet not necessarily share any semantic similarity.
% To circumvent such learning shortcuts,
% Vondrick \etal~\cite{Vondrick18} intentionally drop the color information from the input frames.
% Lai and Xie~\cite{Lai19} further show that a simple channel dropout can be effective.

% With the learnt affinity matrix,
% the downstream dense tracking is therefore posed as mask propagation from $M_{t-1}$~(instance mask of $I_{t-1}$):
% \begin{align}
% M^{i}_t = \sum_{j} A_{ij} M^j_{t-1}
% \label{eq:prop}
% \end{align}

% Note, this architecture design can also be categorized as a simplified version of attention-based models.
% In Transformer~\cite{Vaswani17}, the encoded representations are represented as key-value pairs~(K,V), 
% during decoding, the previous output is compressed into a query~(Q), 
% and the next output is produced by using this query to retrieve relevant information from the set of keys and values.
% While in the aforementioned case for correspondence learning,
% the query~(Q) refers to the pixelwise feature representation computed from the current frame, \ie $f_t$;
% the key~(K) refers to the feature representation of the reference frame, \ie $f_{t-1}$,
% while value~(V) denotes the raw reference frame~($I_{t-1}$) during the training stage, 
% and instance segmentation mask~($M_{t-1}$) during inference.
% For simplicity, we will stick on this set of notations in the following sections.

% ------------------
\subsection{Improved Reconstruction Objective} 
\label{sec:training_signal}
% ------------------
In this section,
we reassess the choices made in previous self-supervised dense tracking works and propose improvements.
%we discuss potential directions for improving training signals in self-supervised dense tracking.
%To analyze the core factors,
For a fair comparison,
we adopt the exact same architecture~(ResNet18) from~\cite{Lai19}.
% ------------------
\vspace{-5pt}
\subsubsection{Decorrelated Color Space}
\label{sec:color}
% ------------------
Extensive experiments in the human visual system have shown that colors can be seen as combinations of the primary colors,
namely red (R), green (G) and blue (B).
For this reason, 
most of the cameras and emissive color displays represent pixels as a triplet of intensities:~$(R,G,B) \in \mathcal{R}^3$.
However, as shown in Figure~\ref{fig:color}, 
a disadvantage of the RGB representation is that the channels tend to be extremely correlated~\cite{Reinhard01}.
In this case, 
the channel dropout proposed in~\cite{Lai19} is unlikely to behave as an effective information bottleneck,
since the dropped channel can almost always be determined by one of the remaining channels.

% ===============
\begin{figure}[!h]
  \centering
  \includegraphics[width=.45\textwidth]{figures/colorspace_v7.pdf}
  \vspace{-2pt}
  \caption{Correlation between channels of RGB and $Lab$ colorspace. 
We randomly take $100000$ pixels from a sequence~(snowboard) in the DAVIS dataset and plot the relative relationships between RGB channels. This phenomena generally holds for all natural images~\cite{Reinhard01}, 
due to the fact that all of the channels include a representation of brightness.
Values are normalized for visualization purposes.}
  \label{fig:color}
\end{figure}
% ===============

To remedy this limitation,
we hypothesize that dropout in the decorrelated representations~(\eg~$Lab$) 
would force the model to learn invariances suitable for self-supervised dense tracking;
\ie if the model cannot predict the missing channel from the observed channels,
it is forced to learn a more robust representation rather than relying on local color information.
%for instance, if the color of one input channel is unpredictable from the others, 
%yet the model is still capable to matching the correspondence and copying colors from a reference frame, 
%it must have learnt more robust representations that are invariant to the low-level colors.
%In Section~\ref{exp:ablation}, 
%we validate our conjecture that channel-wise dropout
%are indeed more effective on input frames represented in the $Lab$ color space,
%which separates luminance and chrominance, resulting in low mutual information.

% ------------------
\vspace{-5pt}
\subsubsection{Classification vs. Regression}
\label{sec:loss}
% ------------------
In the recent literature on colorization and generative models~\cite{Zhang16_Color,Oord16},
colors were quantized into discrete classes and treated as a multinomial distribution,
since generating images or predicting colors from grayscale images is usually a non-deterministic problem, 
\eg the color of a car can reasonably be red or white.
However, this convention is suboptimal for self-supervised learning of correspondences,
as we are not trying to generate colors for each pixel,
but rather, estimate a precise relocation of pixels in the reference frames.
More importantly,
quantizing the colors leads to an information loss that can be crucial for learning high-quality correspondences.

We conjecture that directly optimizing a regression loss between the reconstructed frame~($\hat{I_{t}}$) and real frame~($I_t$) will provide more discriminative training signals.
In this work, the objective $\mathcal{L}$ is defined as the Huber Loss:
\begin{align}
\mathcal{L} = \frac{1}{n} \sum_{i} z_{i}
\end{align}
\vspace{-.3cm}
\noindent where
\begin{align}
 z_{i} =
        \begin{cases}
        0.5 (\hat{\textbf{I}}^i_t - \textbf{I}^i_t)^2, & \text{if } |\hat{\textbf{I}}^i_t - \textbf{I}^i_t| < 1 \\
        |\hat{\textbf{I}}^i_t - \textbf{I}^i_t| - 0.5, & \text{otherwise }
        \end{cases}
\end{align}
where $\hat{\textbf{I}}^i_t$ refers to the pixel (a vector of $3$ values indicating RGB 
or Lab channels, normalized to the range [-1,1]) in the reconstructed frame that is copied from pixels in the reference frame~$I_{t-1}$,
and $I_t$ is the real frame at time point $t$.

% ------------------

\begin{figure*}[!htb]
  \centering
%  % Requires \usepackage{graphicx}
  \includegraphics[width=.95\textwidth]{figures/scheme_v10.pdf}
  \vspace{-3pt}
  \caption{Structure of MAST. 
  The current frame is used to compute \textbf{query} to attend and retrieve from memory (\textbf{key} \& \textbf{value}). 
  During training, we use raw video frame as \textbf{value} for self-supervision. 
  Once the encoder is trained, we use instance mask as \textbf{value}. See Section~\ref{sec:memory} for details.}
  \vspace{-5pt}
  \label{fig:scheme}
\end{figure*}
% ------------------

\vspace{5pt}
\subsection{Memory-augmented Tracking}
\label{sec:memory}
% {\color{red} Todo: transition}
So far we have discussed the straightforward attention-based mechanism for propagating
a mask from a single previous frame.
However, as predictions are made recursively,
errors caused by object occlusion and disocclusion tend to accumulate 
and eventually degrade the subsequent predictions.
To resolve this issue, we propose an attention-based tracker that \emph{efficiently} makes use of \emph{multiple} reference frames. 

\subsubsection{Multi-frame tracker}
An overview of our tracking model is shown in Figure~\ref{fig:scheme}.
To summarize the tracking process: given the current frame and multiple past frames (memory bank) as input,
we first compute the query Q from the current frame and a set of key (K), value (V) pairs from the memory frames.
Here we follow the general procedure in previous works as described in Sec.~\ref{sec:background},
where K and Q are computed from a shared-weight feature extractor and
V is equal to the input frame (during training) or object mask (during testing).
The computed affinity between Q and K is then used to make a prediction for each query pixel
based on V.

Note we don't put any weights on the frames,
as this should have been encoded in the affinity matrix, 
\emph{e.g.}~when the two frames are dis-similar due to temporal distance,
the corresponding similarity value will be naturally low,
and its label will have less contribution to the labeling of a target pixel.

The decision of which pixels to include in K is crucial for good performance.
Including all pixels previously seen is far too computationally expensive due to the quadratic explosion of the affinity matrix (\eg
the network of~\cite{Lai19} produces affinity matrices with more than 1 billion elements on 480p videos).
To reduce computation, \cite{Lai19} exploit temporal smoothness in videos
and apply restricted attention, only computing the affinity with pixels in a ROI around the query pixel location.
%The authors show that the method yields better performances and is computationally-efficient - \eg
%reducing size of similarity matrices by two orders of magnitude.
However, the temporal smoothness assumption holds only for temporally near frames.

To efficiently process temporally distant frames, we propose a two-step attention mechanism.
The first stage involves coarse pixel-matching with the frames in the memory bank to
determine ROIs that are likely to contain good matches with the query pixel.
In the second stage, we extract the ROIs and compute fine-grained pixel matching,
as described in Sec.~\ref{sec:background}.
Next, we describe the first coarse-matching stage in greater detail.
Overall, the process can be summarized in Algorithm~\ref{algorithm}.

\setlength{\textfloatsep}{2pt}% Remove \textfloatsep
\begin{algorithm}[!htb]
\small
  \caption{MAST} 
  \begin{algorithmic}[1]
    \State Choose $m$ reference frames $Q_1, Q_2, ... Q_m$
    \State Localize ROI $R_1, R_2, ... R_m$ according to 3.3.2 (Eq. 5 and 6) for each of the reference frames 
    \State Compute \textit{unnormalized} similarity matrix $A^{ij}_t = \langle\ R_t^i,K^j\rangle $  between target frame $K$ and each ROI.
    \State Normalize $A_{1..m}$ so that they altogether sum up to 1. 
    \State Output: pixel's label is determined by aggregating the labels of the ROI pixels (weighted by its affinity score).
  \end{algorithmic} 
\label{algorithm}
\end{algorithm}

%Next, the Query-Key-Value set is used to compute the current prediction with a simple  \textit{two-stage attention} process.
%In the first stage (\textit{ROI Localization}), for every  pixel in Query, we estimate a \textit{region of interest (ROIs)} in each Key. These ROIs represent a region where the  pixel in Query is likely to locate. For example, the football in Fig.~\ref{fig:scheme} to the right of the current frame should find the same football as ROIs in past frames.
% This process is explained in more detail in the section~\ref{sec:localization}.

%In the second stage, we compute a softmaxed similarity between these regions and the pixels in Query. This similarity is then used to retrieve Values from corresponding ROI regions as prediction. This second stage is a simple extension from the basic attention mechanism described in Sec.~\ref{sec:background}: we simply compute a \textit{single} softmax across space and time and sample only from ROIs.


% To resolve this challenge,
% we propose an attention-based model that can retrieve from multiple reference frames~
% (as shown in Figure~\ref{fig:scheme}). This
% allows longer-term correspondence matching for pixels occluded in the previous frame,
% but visible many frames earlier.
% However, this simple extension struggles for high-resolution dense tracking problems (or more generally computer vision problems),
% due to the quadratic explosion of the affinity matrix.
% For instance, when we use same network as~\cite{Lai19},
% the affinity matrix between two consecutive frames~(480p) exceeds dimension $30,000\times 30,000$.
% Processing multiple such affinity matrices is not only computationally unrealistic, but also unnecessary.

% To exploit temporal smoothness in videos,
% restricted attention~ \cite{Lai19} was applied,
% which effectively defines the candidate search region (in K) to be a local window around the query pixel.
% However,
% such restricted attention does not generalize to multiple reference frames further in time,
% as objects can move large distances or become occluded.

% In order to access and retrieve high-resolution information from the memory bank,
% we propose a deformable attention module that consists of ROI localization and fine-grained matching.
% In practice, a memory bank is composed of feature representations~(Keys) from multiple reference frames,
% \ie~$B = \{K_{t-1}, K_{t-2}, \cdots, K_1\}$.
% For each query pixel from the $t$-th frame, the goal is to coarsely filter frames in the memory bank,
% and pool out candidate regions from all reference frames to reconstruct the query pixel.
% =============
%\begin{figure}[!htb]
%  \centering
%  % Requires \usepackage{graphicx}
%  \includegraphics[width=.48\textwidth]{figures/self_attention_v1.pdf}
%  \vspace{-4pt}
%  \caption{Attention functions proposed in \cite{Lai19} and in this work. See text for details.}
%  \label{fig:self_attention}
%\end{figure}
% \vspace{-10pt}
% =============

\subsubsection{ROI Localization}
\label{sec:localization}
The goal of ROI localization is to estimate the candidate windows non-locally from memory banks. As shown in Figure~\ref{fig:ROI}, this can be achieved through restricted attention with varying dilation rate.

Intuitively, for short term memory (temporally close frames),
dilation is not required since spatial-temporal coherence naturally exists in videos;
%thus the $im2col$ falls back to the standard image-to-matrix transformation in ConvNets, 
thus ROI localization becomes restricted attention~(similar to \cite{Lai19}).
However, for long term memory (\eg the first frame),
we aim to account for the fact that objects can potentially appear anywhere in the reference frames.
We unify both scenarios into a single framework for learning ROI localization.
% ===============
\begin{figure}[H]
  \centering
%  % Requires \usepackage{graphicx}
  \includegraphics[width=.4\textwidth]{figures/NCF_v1.pdf}
  \vspace{-3pt}
  \caption{ROI Localization.}
  \label{fig:ROI}
\end{figure}
% ===============

Formally, for the query pixel $i$ in $I_t$ to localize the ROI from frame~($I_{t-N}$),
%the initial process can be described as:
we first compute $H^i_{t-N, x,y}$, the similarity heatmap between $i$ and all candidate pixels in the dilated window,
in parallel:
\begin{align}
H^i_{t-N, x,y} = softmax(Q^i_t \cdot im2col(K^i_{t-N}, \gamma_{t-N}))
\end{align}
where $\gamma_{t-N}$ refers to the dilation rate for window sampling in frame $I_{t-N}$ and $\gamma_{t-N} \propto N$,
and $im2col$ refers to an operation that transforms the input feature map into a matrix based on dilation rate. Specifically, in our experiments, we use $\gamma_{t-N} = \left \lceil (t-N)  / 15 \right \rceil$.

The center coordinates for ROIs can be then computed via a \textit{soft-argmax} operation:
\begin{align}
P^i_{x,y} = \sum_{x,y} H^i_{x,y} * C 
\end{align}
where $P_{xy}$ is the estimated center location of the candidate window in frame $I_{t-N}$ for query pixel $I^i_t$,
and $C$ refers to the grid coordinates~($x,y$) corresponding to the pixels in the window from $im2col$.
The resampled Key~($\hat{K}^i_{t-N}$) for pixel $I^i_t$ can be extracted with a bilinear sampler~\cite{Jaderberg2015}.
With all the candidate Keys dynamically sampled from different reference frames of the memory bank, 
each pixel can therefore emit the fine-grained matching with only these localized Keys,
resembling the standard restricted attention.
Therefore, with the proposed design, 
the memory-augmented model can efficiently access high-resolution information for correspondence matching, 
without incurring large physical memory costs.  

%\subsubsection{Why two-stage process}
%A basic solution for memory retrival is dot-product attention across all reference frames (Eq.~\ref{eq:attention} and \ref{eq:affinity}).
%However, this simple mechanism struggles for high-resolution tracking because of the quadratic explosion of the affinity matrix (\eg
%the network of~\cite{Lai19} produce affinity matrices with more than 1 billion elements on 480p videos).
%Although it allows memory retrival in theory, processing multiple such affinity matrices is simply computationally unrealistic.
%
%To exploit temporal smoothness in videos,
%\cite{Lai19} applies restricted attention,
%effectively placing the ROI around the query pixel.
%The authors show that the method yields better performances and is computationally-efficient - \eg
%reducing size of similarity matrices by two orders of magnitude.
%However,
%such restricted attention only works for close-by frames since large movement cannot be modelled.
%
%To get the best of both worlds, we borrow intuition from the classical coarse-to-fine process.
%The addition of ROI Localization module first coarsely filter frames in the memory bank, which is then processed for  fine-grained matching. By using the same window size, it models large movement without using any extra memory size compared to restricted attention.

% \subsubsection{Tracking from Multi-frames}
% {\color{red} Todo: add this section. explain technical details of making current prediction (\eg how to compute memory, multiple affinity matrix; how to warp multiple frames etc.). }


% \subsubsection{Matching \& Resampling}
% Once the ROIs are selected from multiple reference frames in the memory banks,
% the affinity matrix $A$ can be computed in a similar way to Eq.~\ref{eq:affinity},
% and the query pixel is reconstructed by a linear combination of all the pixels in the ROIs.
% Ideally, as objects can be occluded or disoccluded throughout the video,
% the query pixel will have a better chance of finding correspondences from the reference frames in the memory bank.


%we can use the pixel similarities to determine if the query pixel appears in the frame. 
%If a query pixel does not show up in a frame, the response in the ROI is all low. 
%In contrast, if a query pixel appear in a frame, 
%the response is high. 
%Since we aim to resample the query pixel from all memorized frames, 
%a simple solution is to find the weights to linearly combine the retrieved pixels and reconstruct the query pixel. 
%A natural solution is to find the weight is by applying a softmax acrossing both spatial and temporal dimension.

%\begin{align}
%A_{ijk} =  \frac{exp\langle\ f^i_t,f^j_k\rangle}{\sum_{jk} exp\langle\ f^i_t,f^j_{k}\rangle}
%\end{align}
%where $A$ stands for a similarity volume now.
%If the query pixel does not show up in some frames,
%the similarity of the entire frame is lower and the frame will be automatically ignored by the \textit{softmax} operation.

% \subsubsection{Bidirectional correspondence searching}
% When computing the reconstruction error, 
% the current methods only copy pixels from the previous frames.
% This can cause issues on pixels that are only visible in the curret frame, 
% but \emph{not visible} in any of the previous frames,
% Therefore, it violates the fundamental assumption that each pixel can be matched with pixels in previous frames,
% either introducing a high photometric loss or leading the model to compromise the matching performance, 
% and drift to other pixels in the neighborhood.
% These errors mainly come from two sources: pixels that are occluded or disoccluded, 
% and pixels at the boundary coming into the field of view.

% In fact, despite the time flows uni-directionally in the physical world, 
% there is no reason preventing us from exploring bidirectional correspondences in the videos.
% We can actually solve the aforementioned challenge by defining the loss as the minimum of bidrectional matching:
% \begin{align}
% L_p = min\{ L_{I_{t-1 \rightarrow t}},  L_{I_{t+1 \rightarrow t}} \}
% \end{align} 

%\subsection{Upperbound of Self-supervised Learning.}
%In order to demonstrate the power of self-supervised learning, 
%it is essential to train more powerful models.
%The model should at least be able to overfit the training set, 
%otherwise, we are not taking the core benefit of unsupervised learning.\\

%While checking the Table~3 in the BMVC paper,
%it is possible to outperform the supervised learning model with more diverse videos and models with higher capacity, \eg~ResNet-50, typical examples are.

%\subsection{Effectiveness of Finetuning on Dense Tracking.}
%\hl{Finetune the model with video segmentation masks, plot the relationships between the data for supervision and performance. }
%\vspace{0.5cm}

%\subsection{Instance Segmentation with the Self-supervised Representation}
%\hl{Take the learnt re. }
%\vspace{0.5cm}



% We propose a new attention function based on the restricted attention proposed , called \textit{deformable attention}. As shown in fig~\ref{fig:self_attention}, the new attention adds a component called \textit{ROI selection}, which estimate an offset from the given input. 


% Tracker drift remains a fundamental challenge for self-supervised dense tracking.
% As predictions are made recursively,
% errors caused by object occlusion and disocclusion tend to accumulate, 
% and eventually contaminate the subsequent predictions.
% In~\cite{Lai19},
% the authors proposed to alleviate the problem using scheduled sampling and forward-backward cycle consistency.

% In this section,
% we explore other possible solutions, \ie~augmenting the architecture with external memory modules.
% Specifically, we form a space-time non-local correspondence flow between the memory bank and the query image~(as shown in Figure~\ref{fig:scheme}). 
% Ideally, we want to enable each query pixel in the target frame to search all previous frames to find the optimal correspondence,
% however,
% this process is usually intractable as the memory required for computing the affinity matrix will grow quadratically.
% To strike a balance between computational cost and accuracy,
% %To obtain the offset value for each frame, 
% we take inspiration from pre-attentive processing,
% \ie information in previous video frames are coarsely processed to infer an offset for each query pixel, 
% and extract the regions with candidate reference pixels.
% These \emph{small regions} will therefore have the highest salience (a stimulus that stands out the most) or
% relevance to a query pixel, 
% and be bilinearly resampled from reference frames for attentive processing~(fine-grained correspondence matching).

% As an extension to the process described earlier~(Section~\ref{sec:background}),
% multiple reference frames from both long term~($I_{t-N}$, $N$ refers to the temporal gap)
% and short term memory~($I_{t-1}$) are fed as inputs to reconstruct the target frame~($I_t$).
% In the following sections,
% we describe the two core components that form the non-local correspondence flow:
% \textbf{ROI Localization} and \textbf{Matching \& Resampling}.

% %We then obtain all pixels in the query image by resampling from frames in the memory bank based on feature similarity. 
% %First, we estimate a rough region of interest (ROI), 
% %which is the most possible region that the query pixel resides in the corresponding frames. 
% %Next, instead of generating independent current frame prediction, 
% %we compute a single dot-product similarity volume between all ROIs and the query pixel. 
% %Finally, this volume is softmaxed and the query pixel is resampled as a linear combination
% %(weighted by aforementioned similarities) of pixels in all RoIs.  

% %\subsubsection{Non-local Correspondence Flow}
% %Figure~\ref{fig:Flow} illustrates the augmented correspondence flow, 
% %which is used to reconstruct the current frame with earlier frames. 
% %The non-local correspondence flow extends the correspondence flow with an offset, 
% %so that the representation could be used to model large movements. 
% %Taking two frames as input, ROI Localization first estimate the offset. 
% %A region of interest(ROI) is then extracted with a bilinear sampler at the offset location. 
% %Multiple such ROIs are extracted from several frames in the memory bank and used to match and resample the current pixel. 

% %
% % ===============
% %\begin{figure}[H]
% %  \centering
% %  % Requires \usepackage{graphicx}
% %  \includegraphics[width=.45\textwidth]{figures/flow_v1.pdf}
% %  \vspace{-3pt}
% %  \caption{Non-local Correspondence Flow. See text for details. }
% %  \label{fig:Flow}
% %\end{figure}
% % ===============



==> untitled folder/sec/related.tex <==
%!TEX root=../egpaper_for_review.tex
\section{Related Work}
\par \noindent \textbf{Dense tracking~(\emph{aka.}~semi-supervised video segmentation)}
has typically been approached in one of two ways:
propagation-based or detection/segmentation-based.
The former approaches formulate the dense tracking task as a mask propagation problem from the first frame to the consecutive frames.
To leverage the temporal consistency between two adjacent frames, 
many propagation-based methods often try to establish dense correspondences with optical flow or metric learning~\cite{Khoreva17, Hu17, Hu18, Luiten18, Voigtlaender19}.
However, computing optical flow remains a challenging, yet unsolved problem. 
Our method relaxes the constraint of optical flow's one-to-one brightness constancy constraint and spatial smoothness,
allowing each query pixel to potentially build correspondence with multiple reference pixels. 
On the other hand, 
detection/segmentation-based approaches address the tracking task with sophisticated detection or segmentation networks, 
but since these models are usually not class-agnostic during training,
they often have to be fine-tuned on the first frame of the target video during inference~\cite{Caelles17,Maninis18, Luiten18},
whereas our method requires no fine-tuning. 
\\[-8pt]

\par \noindent \textbf{Self-supervised learning on videos} 
has generated fruitful research in recent years. 
Due to the abundance of online data~\cite{Agrawal15,Denton17,Fernando17, Gan18,Jakab18,Jia16, Lee17, Misra16,Wang15,Wiles18,Wiles18a, Isola15,Jayaraman16,Jayaraman15,Jing18,Kim18,Vondrick18},
various ideas have been explored to learn representations by exploiting the spatio-temporal information in videos.
~\cite{Misra16,Fernando17,Wei18} 
exploit spatio-temporal ordering for learning video representations.
Recently, Han~\etal~\cite{Han19} learn strong video representations for action recognition by self-supervised contrastive learning on raw videos. 
Of more relevance, \cite{Vondrick18, Lai19} have recently leveraged the natural temporal coherency of color in videos, 
to train a network for tracking and correspondence related tasks. We discuss these works in more detail in Section~\ref{sec:background}.
In this work, we propose to augment the self-supervised tracking algorithms with a differentiable memory module.
We also rectify some flaws in their training process.
\\[-8pt]

\par \noindent \textbf{Memory-augmented models}
refer to the computational architecture that has access to a memory repository for prediction.
Such models typically involve an internal memory implicitly updated in a recurrent process, 
\eg LSTM~\cite{Hochreiter97} and GRU~\cite{chung2014empirical}, 
or an explicit memory that can be read or written with an attention-based procedure~\cite{Xu2015,Vaswani17,Bahdanau2015,Wang2018,Devlin18,Kumar2016,Graves2014,Sukhbaatar2015}. 
Memory models have been used for many applications, 
including reading comprehension~\cite{Sukhbaatar2015}, 
summarization~\cite{See2017}, tracking\cite{Zhu17}, video understanding\cite{Wu19}, and
image and video captioning~\cite{Xu2015,Yao2015}. 
In dense visual tracking, 
the popular memory-augmented models treat key frames as memory~\cite{Seoung19}, 
and use attention mechanisms to read from the memory.
Despite its effectiveness, 
the process of computing attention either does not scale to multiple frames or is unable to process high-resolution frames, 
due to the computational bottleneck in hardware, \eg~physical memory.
In this work,
we propose a scalable way to process high-resolution information in a coarse-to-fine manner.
The model enables dynamic localization of salient regions, 
and fine-grained processing is only required for a small fraction of the memory bank.


% Attention-based model
% has recently been adopted as an successful alternative to recurrent neural networks (RNN) as a method for sequence modelling, 
% yielding state-of-the-art performance in language processing and computer vision~(\eg~\cite{Bahdanau2015,Wang2018,Vaswani17,Seoung19,Devlin18}). 
% Attention mechanisms are known to have relatively low computational complexity, 
% are easier to parallelize and also allow for shorter paths between input and output positions, 
% all of which are especially important for the tracking task.
% The first two features enable the required fast computation, 
% while the latter makes it easier to model long-range dependencies, 
% so as to reduce the infamous drift problem.
% %A very recent work~\cite{Seoung19} adopts a similar mechanism for dense tracking,
% %and trains with a large-scale supervised learning.
% In our proposed architecture, we aim to inherit all these desirable properties,
% and design a deformable attention mechanism to access and retrieve high-resolution information from large memory banks.
% \\[-10pt]

% \par \noindent \textbf{Optical flow} falls in another line of relevant research.
% Specifically, in unsupervised learning for optical flow~\cite{Yu16,Wang18,Meister18},
% the goal is to learn a 2D pixel displacement between consecutive frames based on brightness constancy and spatial smoothness.
% This leads to the popular photometric loss which measures the difference between the reference image and the warped image.
% At first glance, our proposed self-supervised correspondence learning may seem very similar to optical flow.
% However, there exist two fundamental differences:
% first, optical flow usually assumes one-to-one mappings between pixels in subsequent frames; 
% therefore, the number of pixels belonging to the objects will neither increase nor decrease,
% causing problems when tracking objects under large scale variations, occlusions, and disocclusions.
% Second, the correspondence learning in optical flow is entirely based on low-level color cues.
% In contrast, the proposed self-supervised learning approach targets representations which enable higher level and more robust correspondence learning.

==> untitled folder/sec/teaser.tex <==
% %!TEX root=../egpaper_for_review.tex


% \begin{table}[htbp]
% \centering
% \small
% \begin{tabular}{cccccc}
% \hline
% Methods    & Arch    & Supervised      & Dataset       & Speed     & J\& F        \\ \hline
% Methods    & Arch    & Supervised      & Dataset       & Speed     & J\& F

% \end{tabular}
% \caption{To be filled in.}\label{table:teaser}
% \end{table}

==> untitled folder/supp_sec.tex <==
% ------------------------------------------
\clearpage
\begin{appendices}


\section{Network architecture}
In the same way as CorrFlow~\cite{Lai19}, we use a modified ResNet-18~\cite{He16} architecture. Details of the network are illustrated in Table~\ref{table:network-detail}.
% ==============================
\begin{table}[h!]
\centering
% \scriptsize
\footnotesize\addtolength{\tabcolsep}{5pt}
% \setlength{\extrarowheight}{1pt}

\begin{tabular}{ccc}

 \toprule
 Stage & Output & Configuration \\
 \hline
 0 & $H\times W$ & Input image  \\
  conv1 & $H/2\times W/2$ & $7 \!\times\! 7$, 64, stride 2  \\
  conv2 & $H/2\times W/2$ &
$\begin{bmatrix}
3\times 3, 64 
\\ 
3\times 3, 64 
\end{bmatrix} \times2$ \\
  conv3 & 
$H/4\times W/4$ & 
  $\begin{bmatrix}
3\times 3, 128 
\\ 
3\times 3, 128
\end{bmatrix} \times2$  \\
  conv4 & $H/4\times W/4$ &
 
  $\begin{bmatrix}
3\times 3, 256 
\\ 
3\times 3, 256
\end{bmatrix} \times2$  \\
  conv5 & $H/4\times W/4$ & 
  $\begin{bmatrix}
3\times 3, 256 
\\ 
3\times 3, 256
\end{bmatrix} \times2$  \\

\bottomrule
\end{tabular}
\caption{Network architecture. Residual Blocks are shown in brackets (a residually connected sequence of operations). See \cite{He16} for details.
\label{table:network-detail}}
\end{table}
% ==============================

\section{Optimal memory size}
In Figure~\ref{fig:mem_perf},
we explicitly show the effectiveness of increasing the number of reference frames in the memory bank, 
and confirm that a 5-frame memory is optimal for our task.
% ==============================
\begin{figure}[H]
  \centering
  \includegraphics[width=.45\textwidth]{figures/fig_mem_v1.pdf}
  \vspace{-2pt}
  \caption{\textbf{Optimal memory size}: 
  Here, we test a changing memory size of $n+m$: $n$ short term memory and $m$ long term memory, where $n$ and $m$ grow alternatively. The performance of our model initially increases as the number of frames in memory grows, eventually plateauing at 5 frames. }
  \label{fig:mem_perf}
\end{figure}
% ==============================

\section{Analysis by attributes}
We provide a more detailed accuracy list broken down by video attributes provided by the DAVIS benchmark~\cite{Perazzi16} (listed in Table~\ref{table:attributes}). 
The attributes illustrate the difficulties associated with each video sequence. Figure~\ref{fig:attributes} contains the accuracies categorized by attribute. 
Several trends emerge: \emph{first,} MAST outperforms all other self-supervised and unsupervised models by a large margin in all attributes. 
This shows that our model is robust to various challenges in dense tracking. 
\emph{Second,} MAST obtains significant gains on occlusion-related video sequences (\eg~OOC, OV), 
suggesting that memory-augmentation is a key enabler for high-quality tracking: 
retrieving occluded objects from previous frames is very difficult without memory augmentation. 
\emph{Third,} in videos involving background clutter, \ie background and foreground share similar colors, 
MAST obtains a relatively small improvement over previous methods. 
We conjecture this bottleneck could be caused by a shared photometric loss; 
thus a different loss type (\eg~based on texture consistency) could further improve the result.

% ==============================
\begin{table}[H]
\centering
\footnotesize\addtolength{\tabcolsep}{-1pt}
\begin{tabular}{cc|cc}
\toprule
ID  &  Description & ID  &  Description \\
\midrule
AC    &  Appearance Change   &   IO    &  Interacting Objects \\
BC    &  Background Clutter   &   LR    &  Low Resolution \\
CS    &  Camera-Shake   &   MB    &  Motion Blur  \\
DB    &  Dynamic Background   &   OCC    &  Occlusion  \\
DEF    &  Deformation   &   OV    &  Out-of-view  \\
EA    &  Edge Ambiguity   &   ROT    &  Rotation \\
FM    &  Fast-Motion   &   SC    &  Shape Complexity \\
HO    &  Heterogeneus Object  &   SV    &  Scale-Variation  \\
\bottomrule
\end{tabular}
\caption{List of video attributes provided in the DAVIS benchmark. We break down the validation accuracy according to the attribute list.}
\label{table:attributes}
\end{table}
% ==============================
\begin{figure*}[!htb]
  \centering
 % Requires \usepackage{graphicx}
  \includegraphics[width=1.0\textwidth]
    {figures/attribute_cvpr_v2.pdf}%\bigskip% ... an image
%  \vspace{-20pt}

  \captionof{figure}{\textbf{Accuracy broken down by attribute:} MAST outperforms previous self-supervised methods by a significant margin on all attributes, demonstrating the robustness of our model.}

  \label{fig:attributes}
% \vspace{-1em}
\end{figure*}
% ==============================

\section{YouTube-VOS 2019 dataset}
We also evaluate MAST and two other self-supervised methods on YouTube-VOS 2019 validation dataset. The numerical results are reported in Table~\ref{table:youtube_19}. Augmenting on the 2018 version, the 2019 version contains more videos and object instances. We observe similar trend as reported in the main paper (\ie significant improvement and lower generalization gap).
% ===============
\input{tables/youtube-vos-19.tex}
% ===============

\section{More qualitative results}
As shown in Figure \ref{fig:qualitative}, we provide more qualitative results exhibiting some of difficulties in the tracking task. 
These difficulties include tracking multiple similar objects (multi-instance tracking often fails by conflating similar objects), 
large camera shake (objects may have motion blur), inferring unseen object pose of objects, and so on. 
As shown in the figure, MAST handles these difficulties well.

% ==============================
\begin{figure*}[!htb]
  \centering
 % Requires \usepackage{graphicx}
  \includegraphics[width=\textwidth]{figures/qualitative_more_v1.pdf}
  %\vspace{-15pt}
  \captionof{figure}{\textbf{More qualitative results}  from our \emph{self-supervised dense tracking model} on the YouTube-VOS dataset. 
The number on the top left refers to the frame number in the video. Row 1: Tracking multiple similar objects with scale change. Row 2: Occlusions and out-of-scene objects (hand, bottle, and cup). Row 3: Large camera shake. Row 4: Small object with fine details. Row 5: Inferring unseen pose of the deer; out-of-scene object (hand).}
\label{fig:qualitative}
  \vspace{2em}
\end{figure*}
% ==============================

%\section{Supplementary video}
%In order to better illustrate our results, we provide a supplementary video \texttt{611\_sup\_video.mp4}. In the video, we give simple description of our method and also qualitative comparison with other self-supervised algorithms. We obtain qualtitative results of Video Colorization\cite{Vondrick18} from our reimplementation (our reimplemented achieves 34.1 in $\mathcal{J}$\&$\mathcal{F}$(Mean) while the original paper reports 34.0). The qualitative results for CycleTime\cite{Wang19} and CorrFlow\cite{Lai19} comes from their official codes.

\end{appendices}

==> untitled folder/tables/ablation.tex <==
%!TEX root=../egpaper_for_review.tex

\begin{table*}[t]
\centering
% \footnotesize
\footnotesize\addtolength{\tabcolsep}{-1pt}
\vspace{-5pt}
\begin{minipage}{.3\textwidth}
\centering
\begin{tabular}{cccc}

\toprule
Colors.  & Loss & $\mathcal{J}$(Mean)  & $\mathcal{F}$(Mean) \\
\midrule
\multirow{2}{*}{RGB}   &  Cls.  & 42.5  & 45.3       \\
   &  Reg.  & 52.7  & 57.1       \\
\midrule

 \multirow{2}{*}{HSV} &  Cls.    & 32.5 & 35.3  \\
  &  Reg.    & 54.3 & 58.6  \\

\midrule

\multirow{2}{*}{Lab}  &  Cls.   & 47.1 & 48.9 \\ 
 &  Reg.  & \textbf{61.2}  & \textbf{66.3}\\ 
% \midrule
% Lab   & RGB     & \textbf{61.2}  & \textbf{66.3}       \\ 
% RGB   & Lab     & \textbf{61.2}  & \textbf{66.3}       \\ 
        % Lab+HSV    & todo & todo                     \\
        % Lab+HSV+RGB & todo & todo                     \\

        \bottomrule

\end{tabular}
\vspace{-8pt}
\caption{\textbf{Training colorspaces and loss}: Our final model trained with Lab colorspace with regression loss outperforms all other models on dense tracking task. Higher values are better. }
\label{tab:abl_color}
\end{minipage} \hfill
%
\begin{minipage}{.3\textwidth}
\centering
\vspace{-1pt}
\begin{tabular}{cccc}
\toprule
Input  &  Loss & $\mathcal{J}$(Mean)  & $\mathcal{F}$(Mean) \\
\midrule
Lab   & RGB     & 48.2  & 52.0       \\ 
RGB   & Lab     & 46.8  & 49.9       \\ 
\midrule
Lab   & Lab     & \textbf{61.2}  & \textbf{66.3}    \\
        \bottomrule

        % Lab+HSV    & todo & todo                     \\
        % Lab+HSV+RGB & todo & todo                     \\
\end{tabular}
\vspace{25pt}
\caption{\textbf{Cross color space matching \textit{vs.} single color space}: Cross color space matching shows inferior results compared to single color space.}
\label{tab:abl_cross_color}
\end{minipage} \hfill
%
\begin{minipage}{.3\textwidth}
\centering
\begin{tabular}{ccc}
        \toprule
        I-F Align  & $\mathcal{J}$(Mean)  & $\mathcal{F}$(Mean)   \\ \midrule

        No        & 59.1  & 64.0        \\
        Yes       & \textbf{61.2}  & \textbf{66.3}      \\ 
        \midrule
         & $+2.1$ & $+2.3$  \\
                 \bottomrule

\end{tabular}
\vspace{28pt}
\caption{\textbf{Image-Feature alignment}: Using the improved Image-Feature alignment implementation improves the results. Higher values are better. }
\label{tab:abl_align}
\end{minipage} \hfill
%
\vspace{5pt}
\begin{minipage}{.3\textwidth}
\centering
    \vspace{5pt}

    \begin{tabular}{cccc}
    % \vspace{5pt}
        \toprule 
        Memory  & $\mathcal{J}$(Mean)  & $\mathcal{F}$(Mean)   \\ 

        \midrule

        Only long   &  44.6 & 48.7 \\
        Only short    & 57.3 & 61.8   \\
        \midrule
        
        Both      & \textbf{61.2}  & \textbf{66.3}  \\

         \bottomrule
  
    \end{tabular}
    \vspace{-5pt}
    \caption{\textbf{Memory length}: Removing either long term or short term memory results in a performance drop.
 }

\label{tab:abl_mem}
\vspace{10pt}
\end{minipage}\hfill
\begin{minipage}{.3\textwidth}
\centering
\vspace{6pt}
\begin{tabular}{ccc}

        \toprule
        Propagation  & $\mathcal{J}$(Mean)  & $\mathcal{F}$(Mean)   \\ \midrule

        Soft        & 57.0  & 61.7        \\
        Hard       & \textbf{61.2}  & \textbf{66.3}      \\ 
        \midrule
         & $+4.2$ & $+4.6$  \\
                 \bottomrule

\end{tabular}
\vspace{-4pt}
\caption{\textbf{Soft \textit{vs.} hard propagation}: \textit{Quantizing} class probability of each pixel (hard propagation) shows large gains over propagating probility distribution (soft propagation). }
\label{tab:abl_prop}
\end{minipage} \hfill
%
\begin{minipage}{.35\textwidth}
\centering
    \vspace{6pt}

    \begin{tabular}{ccc}
    \toprule
    Dataset  & $\mathcal{J}$(Mean)  & $\mathcal{F}$(Mean)  \\ 
    \midrule
    OxUvA       & 61.2  & 66.3    \\
    ImageNet VID         & 60.0 & 63.9    \\ 
    YouTube-VOS (w/o anno.)    & 63.3 & 67.6 \\
            \bottomrule

    \end{tabular}
    \vspace{0pt}
    \caption{\textbf{Training dataset}: All datasets provide reasonable performance, with O and Y slightly superior. We conjecture that our model gains from higher quality videos and larger object classes in these datasets. }
\label{tab:abl_dataset}
\end{minipage}
\vspace{-0.2cm}
\end{table*}



==> untitled folder/tables/ablation_0.tex <==
%!TEX root=../egpaper_for_review.tex
\begin{table*}
\centering
% \footnotesize
\footnotesize\addtolength{\tabcolsep}{-1pt}
\begin{minipage}{.3\textwidth}
\centering

\begin{tabular}{ccc}

        \toprule
        I-F Align  & $\mathcal{J}$(Mean)  & $\mathcal{F}$(Mean)   \\ \midrule

        No        & 59.1  & 64.0        \\
        Yes       & \textbf{61.2}  & \textbf{66.3}      \\ 
        \midrule
         & $+2.1$ & $+2.3$  \\
        \bottomrule

\end{tabular}
\caption{Effect of training colorspaces on dense tracking. Plus sign denote multiple training signals. Higher values are better. }

\end{minipage} \hfill
\begin{minipage}{.35\textwidth}
\centering

    \begin{tabular}{cccc}

        \toprule
        Memory  & agg. & $\mathcal{J}$(Mean)  & $\mathcal{F}$(Mean)   \\ \midrule


        Only long 	&  \xmark  & 				   \\
        \midrule
        Only short  &  \xmark  &  &   \\
        % Only short term    &  \cmark    & 57.3 & 61.8   \\
        \midrule
        Both    &  ave  & -  & -      \\
        Both    &  max  & \textbf{61.2}  & \textbf{66.3} \\
        Both    &  ST  & \textbf{61.2}  & \textbf{66.3}    
              \\ 
        \bottomrule

    \end{tabular}
    \caption{Effect of training colorspaces on dense tracking. Plus sign denote multiple training signals. Higher values are better. }

\end{minipage}
\begin{minipage}{.3\textwidth}
\centering

\begin{tabular}{ccc}

        \toprule
        Propagation  & $\mathcal{J}$(Mean)  & $\mathcal{F}$(Mean)   \\ \midrule

        Soft        & 59.1  & 64.0        \\
        Hard       & \textbf{61.2}  & \textbf{66.3}      \\ 
        \midrule
         & $+2.1$ & $+2.3$  \\
        \bottomrule

\end{tabular}
\caption{\textbf{Propagating soft prob. \textit{vs.} hard max}: Effect of training colorspaces on dense tracking. Plus sign denote multiple training signals. Higher values are better. }

\end{minipage} \hfill
\begin{minipage}{.6\textwidth}
\centering

\begin{tabular}{cccccc}

\toprule
Colors.  & Loss & $\mathcal{J}$(Mean)  & $\mathcal{J}$(Recall) & $\mathcal{F}$(Mean)  & $\mathcal{F}$(Recall) \\
\midrule
\multirow{2}{*}{RGB}   &  Cls.  & 52.7  & 57.1       \\
   &  Reg.  & 52.7  & 57.1       \\
\midrule

 \multirow{2}{*}{HSV} &  Cls.    & 54.3 & 58.6  \\
  &  Reg.    & 54.3 & 58.6  \\

\midrule

\multirow{2}{*}{Lab}  &  Cls.   & \textbf{61.2}  & \textbf{66.3}\\ 
 &  Reg.  & \textbf{61.2}  & \textbf{66.3}\\ 

\bottomrule

\end{tabular}
\caption{\textbf{Training colorspaces and loss}: Our final model trained with Lab colorspace with regression loss outperforms all other models on dense tracking task. Higher values are better. }

\end{minipage} \hfill
\begin{minipage}{.3\textwidth}
\centering

\begin{tabular}{cccc}
\toprule
Input  &  Loss & $\mathcal{J}$(Mean)  & $\mathcal{F}$(Mean) \\
\midrule
Lab   & RGB     & \textbf{61.2}  & \textbf{66.3}       \\ 
RGB   & Lab     & \textbf{61.2}  & \textbf{66.3}       \\ 
\midrule
Lab   & Lab     & \textbf{61.2}  & \textbf{66.3}       \\ 
        % Lab+HSV    & todo & todo                     \\
        % Lab+HSV+RGB & todo & todo                     \\

        \bottomrule

\end{tabular}
\caption{\textbf{Cross color space matching \textit{vs.} single color space}: Effect of training colorspaces on dense tracking. Plus sign denote multiple training signals. Higher values are better. }

\end{minipage} \hfill
% \begin{minipage}{.35\textwidth}
% \centering

%     \begin{tabular}{ccc}
%     \toprule
%     Dataset  & $\mathcal{J}$(Mean)  & $\mathcal{F}$(Mean)  \\ 
%     \midrule

%     VID         & 60.0 & 63.9    \\ 
%     Kinetics    & todo & todo           \\
%     OxUvA       & 61.2  & 66.3    \\

%     \bottomrule
%     \end{tabular}
%     \caption{Effect of training colorspaces on dense tracking. Plus sign denote multiple training signals. Higher values are better. }

% \end{minipage}
\end{table*}



==> untitled folder/tables/color.tex <==
%!TEX root=../egpaper_for_review.tex

% ===============
\begin{table}[h]
\centering
\footnotesize\addtolength{\tabcolsep}{-5pt}
\begin{tabular}{c @{\extracolsep{\fill}} ccccc}
\toprule
Colorspace  & $\mathcal{J}$(Mean)  & $\mathcal{F}$(Mean) &  \\ \midrule

Lab        & 61.2  & 66.3       \\ 
RGB        & 52.7  & 57.1       \\
HSV        & 54.3 & 58.6                     \\
% Lab+HSV    & todo & todo                     \\
% Lab+HSV+RGB & todo & todo                     \\
  
\bottomrule
\end{tabular}
\vspace{-8pt}
\caption{Effect of training colorspaces on dense tracking. Plus sign denote multiple training signals. Higher values are better. }
\label{table:color_1}
\end{table}


==> untitled folder/tables/davis-2017.tex <==
%!TEX root=../egpaper_for_review.tex

% ===============
\begin{table*}[!htb]
\centering
\footnotesize\addtolength{\tabcolsep}{-5pt}
\begin{tabular*}{\textwidth}{c @{\extracolsep{\fill}} ccccccccc}
\toprule
Method & Backbone & Supervised & Dataset (Size) & $\mathcal{J}$\&$\mathcal{F}$(Mean) $\uparrow$ & $\mathcal{J}$(Mean) $\uparrow$ & $\mathcal{J}$(Recall) $\uparrow$ & $\mathcal{F}$(Mean) $\uparrow$ & $\mathcal{F}$(Recall) $\uparrow$ \\ \midrule

Vid. Color.~\cite{Vondrick18}  & ResNet-18 & \xmark   & Kinetics (800 hours) & 34.0 & 34.6 & 34.1 & 32.7 & 26.8\\
CycleTime$^\dagger$~\cite{Wang19} & ResNet-50  & \xmark   & VLOG (344 hours) & 48.7 & 46.4 & 50.0 & 50.0 & 48.0  \\
% CycleTime (ResNet-50)~\cite{Wang19} & \xmark   & VLOG (144k videos,  344 hours) & 40.7 & 41.9 & 40.9 & 39.4 & 33.6 \\
% {CorrFlow (ResNet-18)~\cite{Lai19}}                  & \xmark   & Kinetics (300k videos,  800 hours) & {49.5} & {47.7} & {53.2} & {51.3} & {56.5} \\  
CorrFlow$^\dagger$~\cite{Lai19} & ResNet-18  & \xmark   & OxUvA (14 hours) & {50.3} & {48.4} & {53.2} & {52.2} & {56.0} \\
UVC$^\star$~\cite{Li19} & ResNet-18  & \xmark   & Kinetics (800 hours) & {59.5} & {57.7} & {68.3} & {61.3} & {69.8} \\
\textbf{MAST (Ours)} & ResNet-18 & \xmark   & OxUvA (14 hours)  & \textbf{63.7} & \textbf{61.2} & \textbf{73.2} & \textbf{66.3} & \textbf{78.3} \\
\textbf{MAST (Ours)} & ResNet-18 & \xmark   & YT-VOS (5.58 hours)  & \textbf{65.5} & \textbf{63.3} & \textbf{73.2} & \textbf{67.6} & \textbf{77.7} \\
\midrule
ImageNet~\cite{He16} & ResNet-50 & \cmark  & I (1.28M, 0) & 49.7 & 50.3 & - & 49.0 & - \\
OSMN~\cite{Yang18} & VGG-16 & \cmark  & ICD (1.28M, 227k) & 54.8 & 52.5 & 60.9& 57.1 & 66.1 \\
SiamMask~\cite{Wang19a} & ResNet-50 & \cmark  & IVCY (1.28M,  2.7M) & 56.4 & 54.3 & 62.8 & 58.5 & 67.5\\
OSVOS~\cite{Caelles17}   &  VGG-16 & \cmark  & ID (1.28M, 10k) & 60.3 & 56.6 & 63.8 & 63.9 & 73.8     \\
%VideoMatch~\cite{Hu18}   & \cmark  & I+C+D & 62.4  & 56.5 & - & 68.2 & -     \\
OnAVOS~\cite{Voigtlaender17}  & ResNet-38  & \cmark  & ICPD (1.28M, 517k) & 65.4 & 61.6 & 67.4 & 69.1 & 75.4     \\
OSVOS-S~\cite{Maninis18}& VGG-16 & \cmark  & IPD (1.28M, 17k) & 68.0 & 64.7 & 74.2 & 71.3 & 80.7     \\
FEELVOS~\cite{Voigtlaender19} & Xception-65 &\cmark  & ICDY (1.28M, 663k) & 71.5 &69.1 &79.1 & 74.0 & 83.8     \\
PReMVOS~\cite{Luiten18} & ResNet-101 &\cmark  & ICDPM (1.28M, 527k) & 77.8 & 73.9 & 83.1 & 81.8 & 88.9     \\
STM~\cite{Seoung19} & ResNet-50 &\cmark  & IDY (1.28M, 164k) & 81.8 & 79.2 & - & 84.3 & -     \\
\bottomrule
\end{tabular*}
\vspace{-8pt}
\caption{Video segmentation results on DAVIS-2017 validation set. 
Dataset notations:
I=ImageNet, 
V = ImageNet-VID,
C=COCO, D=DAVIS, 
M=Mapillary,
P=PASCAL-VOC
Y=YouTube-VOS. For size of datasets, we report (length of \textit{raw videos}) for self-supervised methods and (\#image-level annotations, \#pixel-level annotations) for supervised methods. 
$^\star$ denotes concurrent work. $^\dagger$ denotes highest results reported after original publication. Higher values are better. }
\label{table:davis_1}
\end{table*}


==> untitled folder/tables/youtube-vos-19.tex <==
%!TEX root=../supp.tex

% ===============
\begin{table}[!htb]
\centering
\footnotesize\addtolength{\tabcolsep}{-2pt}
\begin{tabular}{c @{\extracolsep{\fill}} ccccccc}
\toprule
% Method & Sup. & Overall & $\mathcal{J}$(Seen) & $\mathcal{F}$(Seen) & $\mathcal{J}$(Unseen) & $\mathcal{F}$(Unseen) \\ 

\multirow{2}{*}{Method} & \multirow{2}{*}{Sup.}  & \multirow{2}{*}{Overall $\uparrow$} & \multicolumn{2}{c}{Seen} & \multicolumn{2}{c}{Unseen} & 
\multirow{2}{*}{Gen. Gap $\downarrow$}\\ 
\cmidrule{4-5} \cmidrule{6-7} 
 &  & & $\mathcal{J}$ $\uparrow$ & $\mathcal{F}$ $\uparrow$ & $\mathcal{J}$ $\uparrow$ & $\mathcal{F}$ $\uparrow$  \\ 

 \midrule

Vid. Color.\cite{Vondrick18}$^\dagger$  &  \xmark & 39.0  & 43.3  & 38.2  & 36.6 & 37.5 & 3.7 \\
CorrFlow\cite{Lai19}  &    \xmark & 47.0   & 51.2   & 46.6 & 44.5  & 45.9 &  3.7 \\
\textbf{MAST~(Ours)}   &  \xmark & \textbf{64.9}  & \textbf{64.3}  & \textbf{65.3}  & \textbf{61.5} & \textbf{68.4} &  \textbf{0.15}\\

\bottomrule
\end{tabular}
\vspace{-8pt}
\caption{Video segmentation results on Youtube-VOS 2019 dataset. Higher values are better. $^\dagger$ indicates results based on our reimplementation.}
\label{table:youtube_19}
\vspace{-2em}
\end{table}


==> untitled folder/tables/youtube-vos.tex <==
%!TEX root=../egpaper_for_review.tex

% ===============
\begin{table}[!htb]
\centering
\footnotesize\addtolength{\tabcolsep}{-2pt}
\begin{tabular}{c @{\extracolsep{\fill}} ccccccc}
\toprule
% Method & Sup. & Overall & $\mathcal{J}$(Seen) & $\mathcal{F}$(Seen) & $\mathcal{J}$(Unseen) & $\mathcal{F}$(Unseen) \\ 

\multirow{2}{*}{Method} & \multirow{2}{*}{Sup.}  & \multirow{2}{*}{Overall $\uparrow$} & \multicolumn{2}{c}{Seen} & \multicolumn{2}{c}{Unseen} & 
\multirow{2}{*}{Gen. Gap $\downarrow$}\\ 
\cmidrule{4-5} \cmidrule{6-7} 
 &  & & $\mathcal{J}$ $\uparrow$ & $\mathcal{F}$ $\uparrow$ & $\mathcal{J}$ $\uparrow$ & $\mathcal{F}$ $\uparrow$  \\ 

 \midrule

Vid. Color.\cite{Vondrick18}$^\dagger$  &  \xmark & 38.9  & 43.1  & 38.6  & 36.6 & 37.4 & 3.9 \\
CorrFlow\cite{Lai19}  &    \xmark & 46.6   & 50.6   & 46.6 & 43.8  & 45.6 &  3.9 \\
\textbf{MAST (Ours)}   &  \xmark & \textbf{64.2}  & \textbf{63.9}  & \textbf{64.9}  & \textbf{\textcolor{blue}{60.3}} & \textbf{\textcolor{blue}{67.7}} &  \textbf{0.4}\\
\midrule

OSMN\cite{Yang18}   & \cmark &  51.2  & 60.0 & 60.1 & 40.6  & 44.0  &  17.75\\
MSK\cite{Khoreva16}    & \cmark &  53.1  & 59.9  & 59.5  & 45.0  & 47.9 &  13.25 \\
RGMP\cite{Oh18}  & \cmark &  53.8  & 59.5  & -  & 45.2  & - &  14.3\\
OnAVOS\cite{Voigtlaender17}  & \cmark &  55.2  & 60.1  & 62.7  & 46.6  & 51.4 &  12.4\\
RVOS\cite{Ventura_2019_CVPR}  & \cmark &  56.8  & 63.6  & 67.2  & 45.5  & 51.0 &  17.15\\
OSVOS\cite{Caelles17}  & \cmark &  58.8  & 59.8  & 60.5  & 54.2  & 60.7 &  2.7\\
S2S\cite{Xu18}  & \cmark &  64.4  & 71.0  & 70.0  & 55.5  & 61.2 &  12.15\\
PreMVOS\cite{Luiten18}  & \cmark &  66.9  & 71.4  & 75.9  & 56.5  & 63.7 &  13.55\\
STM\cite{Seoung19}  & \cmark &  79.4  & 79.7  & 84.2  & \textcolor{red}{72.8}  & \textcolor{red}{80.9} &  5.1\\

\bottomrule
\end{tabular}
\vspace{-5pt}
\caption{Video segmentation results on Youtube-VOS dataset. Higher values are better. According to the evaluation protocol of the benchmark, we report performance separated into ``seen'' and ``unseen'' classes (``Seen'' with respect to training set). $^\dagger$ indicates results based on our reimplementation. The first- and second-best results on the unseen category are highlighted in red and blue, respectively.}
\label{table:youtube_1}
\end{table}

